Stochastic Primal-Dual Three Operator Splitting Algorithm with Extension to Equivariant Regularization-by-Denoising

In this work we propose a stochastic primal-dual three-operator splitting algorithm (TOS-SPDHG) for solving a class of convex three-composite optimization problems. Our proposed scheme is a direct three-operator splitting extension of the SPDHG algorithm [Chambolle et al. 2018]. We provide theoretical convergence analysis showing ergodic $O(1/K)$ convergence rate, and demonstrate the effectiveness of our approach in imaging inverse problems. Moreover, we further propose TOS-SPDHG-RED and TOS-SPDHG-eRED which utilizes the regularization-by-denoising (RED) framework to leverage pretrained deep denoising networks as priors.

==> backup.tex <==

@inproceedings{chizat2019lazy,
  title={On lazy training in differentiable programming},
  author={Chizat, Lenaic and Oyallon, Edouard and Bach, Francis},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2933--2943},
  year={2019}
}

@inproceedings{ergen2020convex,
  title={Convex geometry of two-layer relu networks: Implicit autoencoding and interpretable models},
  author={Ergen, Tolga and Pilanci, Mert},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={4024--4033},
  year={2020},
  organization={PMLR}
}

@article{richtarik2016parallel,
  title={Parallel coordinate descent methods for big data optimization},
  author={Richt{\'a}rik, Peter and Tak{\'a}{\v{c}}, Martin},
  journal={Mathematical Programming},
  volume={156},
  number={1},
  pages={433--484},
  year={2016},
  publisher={Springer}
}

@article{thibault2007three,
  title={A three-dimensional statistical approach to improved image quality for multislice helical CT},
  author={Thibault, Jean-Baptiste and Sauer, Ken D and Bouman, Charles A and Hsieh, Jiang},
  journal={Medical physics},
  volume={34},
  number={11},
  pages={4526--4544},
  year={2007},
  publisher={Wiley Online Library}
}

@article{condat2013primal,
  title={A primal--dual splitting method for convex optimization involving Lipschitzian, proximable and linear composite terms},
  author={Condat, Laurent},
  journal={Journal of optimization theory and applications},
  volume={158},
  number={2},
  pages={460--479},
  year={2013},
  publisher={Springer}
}

@article{vu2013splitting,
  title={A splitting algorithm for dual monotone inclusions involving cocoercive operators},
  author={V{\~u}, Bằng C{\^o}ng},
  journal={Advances in Computational Mathematics},
  volume={38},
  number={3},
  pages={667--681},
  year={2013},
  publisher={Springer}
}

@article{tang2020fast,
  title={A Fast Stochastic Plug-and-Play ADMM for Imaging Inverse Problems},
  author={Tang, Junqi and Davies, Mike},
  journal={arXiv preprint arXiv:2006.11630},
  year={2020}
}

@article{davis2017three,
  title={A three-operator splitting scheme and its optimization applications},
  author={Davis, Damek and Yin, Wotao},
  journal={Set-valued and variational analysis},
  volume={25},
  number={4},
  pages={829--858},
  year={2017},
  publisher={Springer}
}

@article{guo2021compressing,
  title={Compressing Denoising Networks},
  author={Guo, Yudi},
  journal={Masters Thesis (Supervisor: Junqi Tang and Mike Davies), University of Edinburgh},
  year={2021}
}


@article{scieur2019generalized,
  title={Generalized Framework for Nonlinear Acceleration},
  author={Scieur, Damien},
  journal={arXiv preprint arXiv:1903.08764},
  year={2019}
}

@article{driggs2020spring,
  title={Spring: A fast stochastic proximal alternating method for non-smooth non-convex optimization},
  author={Driggs, Derek and Tang, Junqi and Liang, Jingwei and Davies, Mike and Sch{\"o}nlieb, Carola-Bibiane},
  journal={SIAM Journal on Imaging Sciences (to appear)},
  year={2021}
}

@article{ergen2020training,
  title={Training convolutional relu neural networks in polynomial time: Exact convex optimization formulations},
  author={Ergen, Tolga and Pilanci, Mert},
  journal={arXiv preprint arXiv:2006.14798},
  year={2020}
}

@article{tachella2020neural,
  title={The Neural Tangent Link Between CNN Denoisers and Non-Local Filters},
  author={Tachella, Juli{\'a}n and Tang, Junqi and Davies, Mike},
  journal={IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2021}
}

@article{chen2021equivariant,
  title={Equivariant Imaging: Learning Beyond the Range Space},
  author={Chen, Dongdong and Tachella, Juli{\'a}n and Davies, Mike E},
  journal={ICCV (to appear)},
  year={2021}
}

@article{tang2020practicality,
  title={The practicality of stochastic optimization in imaging inverse problems},
  author={Tang, Junqi and Egiazarian, Karen and Golbabaee, Mohammad and Davies, Mike},
  journal={IEEE Transactions on Computational Imaging},
  volume={6},
  pages={1471--1485},
  year={2020},
  publisher={IEEE}
}


@InProceedings{pilanci2020neural, 
title = {Neural Networks are Convex Regularizers: Exact Polynomial-time Convex Optimization Formulations for Two-layer Networks}, 
author = {Pilanci, Mert and Ergen, Tolga}, booktitle = {Proceedings of the 37th International Conference on Machine Learning}, pages = {7695--7705}, year = {2020}, volume = {119}, series = {Proceedings of Machine Learning Research}, month = {13--18 Jul}, publisher = {PMLR} 
}

@article{niknejad2019external,
  title={External Patch-Based Image Restoration Using Importance Sampling},
  author={Niknejad, Milad and Bioucas-Dias, Jos{\'e} and Figueiredo, M{\'a}rio AT},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={9},
  pages={4460--4470},
  year={2019},
  publisher={IEEE}
}

@article{sahiner2020convex,
  title={Convex Regularization Behind Neural Reconstruction},
  author={Sahiner, Arda and Mardani, Morteza and Ozturkler, Batu and Pilanci, Mert and Pauly, John},
  journal={arXiv preprint arXiv:2012.05169},
  year={2020}
}

@article{tachella2020cnn,
  title={CNN Denoisers As Non-Local Filters: The Neural Tangent Denoiser},
  author={Tachella, Juli{\'a}n and Tang, Junqi and Davies, Mike},
  journal={arXiv preprint arXiv:2006.02379},
  year={2020}
}

@article{sun2020scalable,
  title={Scalable Plug-and-Play ADMM with Convergence Guarantees},
  author={Sun, Yu and Wu, Zihui and Wohlberg, Brendt and Kamilov, Ulugbek S},
  journal={arXiv preprint arXiv:2006.03224},
  year={2020}
}

@article{hansen2018air,
  title={AIR Tools II: algebraic iterative reconstruction methods, improved implementation},
  author={Hansen, Per Christian and J{\o}rgensen, Jakob Sauer},
  journal={Numerical Algorithms},
  volume={79},
  number={1},
  pages={107--137},
  year={2018},
  publisher={Springer}
}

@article{chouzenoux2017stochastic,
  title={A stochastic majorize-minimize subspace algorithm for online penalized least squares estimation},
  author={Chouzenoux, Emilie and Pesquet, Jean-Christophe},
  journal={IEEE Transactions on Signal Processing},
  volume={65},
  number={18},
  pages={4770--4783},
  year={2017},
  publisher={IEEE}
}



@inproceedings{scieur2017nonlinear,
  title={Nonlinear acceleration of stochastic algorithms},
  author={Scieur, Damien and Bach, Francis and d'Aspremont, Alexandre},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3982--3991},
  year={2017}
}

@article{poon2020geometry,
  title={Geometry of First-Order Methods and Adaptive Acceleration},
  author={Poon, Clarice and Liang, Jingwei},
  journal={arXiv preprint arXiv:2003.03910},
  year={2020}
}

@article{chambolle2015convergence,
  title={On the convergence of the iterates of the “fast iterative shrinkage/thresholding algorithm”},
  author={Chambolle, Antonin and Dossal, Ch},
  journal={Journal of Optimization theory and Applications},
  volume={166},
  number={3},
  pages={968--982},
  year={2015},
  publisher={Springer}
}

@article{combettes2015stochastic,
  title={Stochastic quasi-Fej{\'e}r block-coordinate fixed point iterations with random sweeping},
  author={Combettes, Patrick L and Pesquet, Jean-Christophe},
  journal={SIAM Journal on Optimization},
  volume={25},
  number={2},
  pages={1221--1248},
  year={2015},
  publisher={SIAM}
}


@article{zhao2019optimal_a,
  title={Optimal algorithms for stochastic three-composite convex-concave saddle point problems},
  author={Zhao, Renbo},
  journal={arXiv preprint arXiv:1903.01687},
  year={2019}
}

@article{dou2019training,
  title={Training neural networks as learning data-adaptive kernels: Provable representation and approximation benefits},
  author={Dou, Xialiang and Liang, Tengyuan},
  journal={arXiv preprint arXiv:1901.07114},
  year={2019}
}

@article{mei2019generalization,
  title={The generalization error of random features regression: Precise asymptotics and double descent curve},
  author={Mei, Song and Montanari, Andrea},
  journal={arXiv preprint arXiv:1908.05355},
  year={2019}
}

@article{nakkiran2020optimal,
  title={Optimal Regularization Can Mitigate Double Descent},
  author={Nakkiran, Preetum and Venkat, Prayaag and Kakade, Sham and Ma, Tengyu},
  journal={arXiv preprint arXiv:2003.01897},
  year={2020}
}

@article{belkin2019reconciling,
  title={Reconciling modern machine-learning practice and the classical bias--variance trade-off},
  author={Belkin, Mikhail and Hsu, Daniel and Ma, Siyuan and Mandal, Soumik},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={32},
  pages={15849--15854},
  year={2019},
  publisher={National Acad Sciences}
}



@article{shankar2020neural,
  title={Neural Kernels Without Tangents},
  author={Shankar, Vaishaal and Fang, Alex and Guo, Wenshuo and Fridovich-Keil, Sara and Schmidt, Ludwig and Ragan-Kelley, Jonathan and Recht, Benjamin},
  journal={arXiv preprint arXiv:2003.02237},
  year={2020}
}

@inproceedings{williams2001using,
  title={Using the Nystr{\"o}m method to speed up kernel machines},
  author={Williams, Christopher KI and Seeger, Matthias},
  booktitle={Advances in neural information processing systems},
  pages={682--688},
  year={2001}
}

@inproceedings{rahimi2008random,
  title={Random features for large-scale kernel machines},
  author={Rahimi, Ali and Recht, Benjamin},
  booktitle={Advances in neural information processing systems},
  pages={1177--1184},
  year={2008}
}

@inproceedings{mairal2016end,
  title={End-to-end kernel learning with supervised convolutional kernel networks},
  author={Mairal, Julien},
  booktitle={Advances in neural information processing systems},
  pages={1399--1407},
  year={2016}
}

@inproceedings{rudi2017generalization,
  title={Generalization properties of learning with random features},
  author={Rudi, Alessandro and Rosasco, Lorenzo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3215--3225},
  year={2017}
}

@inproceedings{yang2012nystrom,
  title={Nystr{\"o}m method vs random fourier features: A theoretical and empirical comparison},
  author={Yang, Tianbao and Li, Yu-Feng and Mahdavi, Mehrdad and Jin, Rong and Zhou, Zhi-Hua},
  booktitle={Advances in neural information processing systems},
  pages={476--484},
  year={2012}
}

@inproceedings{sinha2016learning,
  title={Learning kernels with random features},
  author={Sinha, Aman and Duchi, John C},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1298--1306},
  year={2016}
}
@inproceedings{wilson2016deep,
  title={Deep kernel learning},
  author={Wilson, Andrew Gordon and Hu, Zhiting and Salakhutdinov, Ruslan and Xing, Eric P},
  booktitle={Artificial Intelligence and Statistics},
  pages={370--378},
  year={2016}
}

@inproceedings{li2019learning,
  title={Learning adaptive random features},
  author={Li, Yanjun and Zhang, Kai and Wang, Jun and Kumar, Sanjiv},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={4229--4236},
  year={2019}
}

@inproceedings{wilson2016stochastic,
  title={Stochastic variational deep kernel learning},
  author={Wilson, Andrew G and Hu, Zhiting and Salakhutdinov, Russ R and Xing, Eric P},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2586--2594},
  year={2016}
}

@inproceedings{chizat2018global,
  title={On the global convergence of gradient descent for over-parameterized models using optimal transport},
  author={Chizat, Lenaic and Bach, Francis},
  booktitle={Advances in neural information processing systems},
  pages={3036--3046},
  year={2018}
}
@article{du2018gradient1,
  title={Gradient descent provably optimizes over-parameterized neural networks},
  author={Du, Simon S and Zhai, Xiyu and Poczos, Barnabas and Singh, Aarti},
  journal={arXiv preprint arXiv:1810.02054},
  year={2018}
}

@inproceedings{gunasekar2017implicit,
  title={Implicit regularization in matrix factorization},
  author={Gunasekar, Suriya and Woodworth, Blake E and Bhojanapalli, Srinadh and Neyshabur, Behnam and Srebro, Nati},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6151--6159},
  year={2017}
}

@inproceedings{du2019graph,
  title={Graph neural tangent kernel: Fusing graph neural networks with graph kernels},
  author={Du, Simon S and Hou, Kangcheng and Salakhutdinov, Russ R and Poczos, Barnabas and Wang, Ruosong and Xu, Keyulu},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5724--5734},
  year={2019}
}

@article{li2019enhanced,
  title={Enhanced Convolutional Neural Tangent Kernels},
  author={Li, Zhiyuan and Wang, Ruosong and Yu, Dingli and Du, Simon S and Hu, Wei and Salakhutdinov, Ruslan and Arora, Sanjeev},
  journal={arXiv preprint arXiv:1911.00809},
  year={2019}
}

@inproceedings{allen2019learning,
  title={Learning and generalization in overparameterized neural networks, going beyond two layers},
  author={Allen-Zhu, Zeyuan and Li, Yuanzhi and Liang, Yingyu},
  booktitle={Advances in neural information processing systems},
  pages={6155--6166},
  year={2019}
}

@inproceedings{li2018learning,
  title={Learning overparameterized neural networks via stochastic gradient descent on structured data},
  author={Li, Yuanzhi and Liang, Yingyu},
  booktitle={Advances in Neural Information Processing Systems},
  pages={8157--8166},
  year={2018}
}
@article{du2018gradient,
  title={Gradient descent finds global minima of deep neural networks},
  author={Du, Simon S and Lee, Jason D and Li, Haochuan and Wang, Liwei and Zhai, Xiyu},
  journal={arXiv preprint arXiv:1811.03804},
  year={2018}
}

@article{woodworth2019kernel,
  title={Kernel and deep regimes in overparametrized models},
  author={Woodworth, Blake and Gunasekar, Suriya and Lee, Jason and Soudry, Daniel and Srebro, Nathan},
  journal={arXiv preprint arXiv:1906.05827},
  year={2019}
}

@article{zhang2019all,
  title={Are all layers created equal?},
  author={Zhang, Chiyuan and Bengio, Samy and Singer, Yoram},
  journal={arXiv preprint arXiv:1902.01996},
  year={2019}
}

@article{malach2020proving,
  title={Proving the Lottery Ticket Hypothesis: Pruning is All You Need},
  author={Malach, Eran and Yehudai, Gilad and Shalev-Shwartz, Shai and Shamir, Ohad},
  journal={arXiv preprint arXiv:2002.00585},
  year={2020}
}

@inproceedings{arora2019exact,
  title={On exact computation with an infinitely wide neural net},
  author={Arora, Sanjeev and Du, Simon S and Hu, Wei and Li, Zhiyuan and Salakhutdinov, Russ R and Wang, Ruosong},
  booktitle={Advances in Neural Information Processing Systems},
  pages={8139--8148},
  year={2019}
}

@inproceedings{lee2019wide,
  title={Wide neural networks of any depth evolve as linear models under gradient descent},
  author={Lee, Jaehoon and Xiao, Lechao and Schoenholz, Samuel and Bahri, Yasaman and Novak, Roman and Sohl-Dickstein, Jascha and Pennington, Jeffrey},
  booktitle={Advances in neural information processing systems},
  pages={8570--8581},
  year={2019}
}

@inproceedings{jacot2018neural,
  title={Neural tangent kernel: Convergence and generalization in neural networks},
  author={Jacot, Arthur and Gabriel, Franck and Hongler, Cl{\'e}ment},
  booktitle={Advances in neural information processing systems},
  pages={8571--8580},
  year={2018}
}

@article{woodworth2019kernel,
  title={Kernel and deep regimes in overparametrized models},
  author={Woodworth, Blake and Gunasekar, Suriya and Lee, Jason and Soudry, Daniel and Srebro, Nathan},
  journal={arXiv preprint arXiv:1906.05827},
  year={2019}
}

@article{fadili2010total,
  title={Total variation projection with first order schemes},
  author={Fadili, Jalal M and Peyr{\'e}, Gabriel},
  journal={IEEE Transactions on Image Processing},
  volume={20},
  number={3},
  pages={657--669},
  year={2010},
  publisher={IEEE}
}

@misc{ozaslan2019regularized,
    title={Regularized Momentum Iterative Hessian Sketch for Large Scale Linear System of Equations},
    author={Ibrahim Kurban Ozaslan and Mert Pilanci and Orhan Arikan},
    year={2019},
    eprint={1912.03514},
    archivePrefix={arXiv},
    primaryClass={math.OC}
}

@article{lacotte2019faster,
  title={Faster Least Squares Optimization},
  author={Lacotte, Jonathan and Pilanci, Mert},
  journal={arXiv preprint arXiv:1911.02675},
  year={2019}
}

@article{rokhlin2008fast,
  title={A fast randomized algorithm for overdetermined linear least-squares regression},
  author={Rokhlin, Vladimir and Tygert, Mark},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={36},
  pages={13212--13217},
  year={2008},
  publisher={National Acad Sciences}
}

@inproceedings{zhao2019optimal,
  title={An Optimal Algorithm for Stochastic Three-Composite Optimization},
  author={Zhao, Renbo and Haskell, William B and Tan, Vincent YF},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={428--437},
  year={2019}
}

@article{rosasco2014convergence,
  title={Convergence of stochastic proximal gradient algorithm},
  author={Rosasco, Lorenzo and Villa, Silvia and V{\~u}, Bang C{\^o}ng},
  journal={arXiv preprint arXiv:1403.5074},
  year={2014}
}

@inproceedings{ulas2017robust,
  title={A Robust Reconstruction Method for Quantitative Perfusion MRI: Application to Brain Dynamic Susceptibility Contrast (DSC) Imaging},
  author={Ulas, Cagdas and Gomez, Pedro A and Sperl, Jonathan I and Preibisch, Christine and Menzel, Marion I and Haase, Axel and Menze, Bjoern H}
}

@article{ulas2017accelerated,
  title={Accelerated Reconstruction of Perfusion-Weighted MRI Enforcing Jointly Local and Nonlocal Spatio-temporal Constraints},
  author={Ulas, Cagdas and Preibisch, Christine and Sperl, Jonathan and Pyka, Thomas and Kalpathy-Cramer, Jayashree and Menze, Bjoern},
  journal={arXiv preprint arXiv:1708.07808},
  year={2017}
}

@inproceedings{musco2018stability,
  title={Stability of the Lanczos method for matrix function approximation},
  author={Musco, Cameron and Musco, Christopher and Sidford, Aaron},
  booktitle={Proceedings of the Twenty-Ninth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={1605--1624},
  year={2018},
  organization={Society for Industrial and Applied Mathematics}
}

@article{needell2014paved,
  title={Paved with good intentions: analysis of a randomized block Kaczmarz method},
  author={Needell, Deanna and Tropp, Joel A},
  journal={Linear Algebra and its Applications},
  volume={441},
  pages={199--221},
  year={2014},
  publisher={Elsevier}
}

@article{tropp2012user,
  title={User-friendly tail bounds for sums of random matrices},
  author={Tropp, Joel A},
  journal={Foundations of computational mathematics},
  volume={12},
  number={4},
  pages={389--434},
  year={2012},
  publisher={Springer}
}

@article{gower2018stochastic,
  title={Stochastic quasi-gradient methods: Variance reduction via Jacobian sketching},
  author={Gower, Robert M and Richt{\'a}rik, Peter and Bach, Francis},
  journal={arXiv preprint arXiv:1805.02632},
  year={2018}
}

@article{tropp2004greed,
  title={Greed is good: Algorithmic results for sparse approximation},
  author={Tropp, Joel A},
  journal={IEEE Transactions on Information theory},
  volume={50},
  number={10},
  pages={2231--2242},
  year={2004}
}

@article{combettes2004image,
  title={Image restoration subject to a total variation constraint},
  author={Combettes, Patrick L and Pesquet, J-C},
  journal={IEEE transactions on image processing},
  volume={13},
  number={9},
  pages={1213--1222},
  year={2004},
  publisher={IEEE}
}

@article{udell2019big,
  title={Why Are Big Data Matrices Approximately Low Rank?},
  author={Udell, Madeleine and Townsend, Alex},
  journal={SIAM Journal on Mathematics of Data Science},
  volume={1},
  number={1},
  pages={144--160},
  year={2019},
  publisher={SIAM}
}




@inproceedings{gazagnadou2019optimal,
  title={Optimal Mini-Batch and Step Sizes for SAGA},
  author={Gazagnadou, Nidham and Gower, Robert and Salmon, Joseph},
  booktitle={International Conference on Machine Learning},
  pages={2142--2150},
  year={2019}
}

@article{nemirovsky1983problem,
  title={Problem complexity and method efficiency in optimization.},
  author={Nemirovsky, Arkadii Semenovich and Yudin, David Borisovich},
  year={1983}
}

@inproceedings{nemirovski1978cesari,
  title={Cesari convergence of the gradient method of approximating saddle points of convex-concave functions},
  author={Nemirovski, Arkadi S and Yudin, David Berkovich},
  booktitle={Doklady Akademii Nauk},
  volume={239},
  number={5},
  pages={1056--1059},
  year={1978},
  organization={Russian Academy of Sciences}
}

@InProceedings{pmlr-v97-qian19b,
  title = 	 {{SGD}: General Analysis and Improved Rates},
  author = 	 {Gower, Robert Mansel and Loizou, Nicolas and Qian, Xun and Sailanbayev, Alibek and Shulgin, Egor and Richt{\'a}rik, Peter},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning},
  pages = 	 {5200--5209},
  year = 	 {2019},
  volume = 	 {97},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Long Beach, California, USA},
  month = 	 {09--15 Jun},
  publisher = 	 {PMLR}
}

@article{lewis2002active,
  title={Active sets, nonsmoothness, and sensitivity},
  author={Lewis, Adrian S},
  journal={SIAM Journal on Optimization},
  volume={13},
  number={3},
  pages={702--725},
  year={2002},
  publisher={SIAM}
}
@article{chambolle2016introduction,
  title={An introduction to continuous optimization for imaging},
  author={Chambolle, Antonin and Pock, Thomas},
  journal={Acta Numerica},
  volume={25},
  pages={161--319},
  year={2016},
  publisher={Cambridge University Press}
}

@book{hosmer2013applied,
  title={Applied logistic regression},
  author={Hosmer Jr, David W and Lemeshow, Stanley and Sturdivant, Rodney X},
  volume={398},
  year={2013},
  publisher={John Wiley \& Sons}
}

@book{horn2012matrix,
  title={Matrix analysis},
  author={Horn, Roger A and Johnson, Charles R},
  year={2012},
  publisher={Cambridge university press}
}

@article{tropp2008conditioning,
  title={On the conditioning of random subdictionaries},
  author={Tropp, Joel A},
  journal={Applied and Computational Harmonic Analysis},
  volume={25},
  number={1},
  pages={1--24},
  year={2008},
  publisher={Elsevier}
}

@article{shalev2011pegasos,
  title={Pegasos: Primal estimated sub-gradient solver for svm},
  author={Shalev-Shwartz, Shai and Singer, Yoram and Srebro, Nathan and Cotter, Andrew},
  journal={Mathematical programming},
  volume={127},
  number={1},
  pages={3--30},
  year={2011},
  publisher={Springer}
}

@inproceedings{venkatakrishnan2013plug,
  title={Plug-and-play priors for model based reconstruction},
  author={Venkatakrishnan, Singanallur V and Bouman, Charles A and Wohlberg, Brendt},
  booktitle={2013 IEEE Global Conference on Signal and Information Processing},
  pages={945--948},
  year={2013},
  organization={IEEE}
}


@article{kamilov2017plug,
  title={A plug-and-play priors approach for solving nonlinear imaging inverse problems},
  author={Kamilov, Ulugbek S and Mansour, Hassan and Wohlberg, Brendt},
  journal={IEEE Signal Processing Letters},
  volume={24},
  number={12},
  pages={1872--1876},
  year={2017},
  publisher={IEEE}
}
@article{romano2017little,
  title={The little engine that could: Regularization by denoising (RED)},
  author={Romano, Yaniv and Elad, Michael and Milanfar, Peyman},
  journal={SIAM Journal on Imaging Sciences},
  volume={10},
  number={4},
  pages={1804--1844},
  year={2017},
  publisher={SIAM}
}

@article{sun2019block,
  title={Block Coordinate Regularization by Denoising},
  author={Sun, Yu and Liu, Jiaming and Kamilov, Ulugbek S},
  journal={arXiv preprint arXiv:1905.05113},
  year={2019}
}

@article{reehorst2018regularization,
  title={Regularization by denoising: Clarifications and new interpretations},
  author={Reehorst, Edward T and Schniter, Philip},
  journal={IEEE Transactions on Computational Imaging},
  volume={5},
  number={1},
  pages={52--67},
  year={2018},
  publisher={IEEE}
}

@article{tang2019randomized,
  title={Randomized structure-adaptive optimization},
  author={Tang, Junqi},
  year={2019},
  publisher={The University of Edinburgh}
}

@article{hansen2012air,
  title={{AIR} tools—a {MATLAB} package of algebraic iterative reconstruction methods},
  author={Hansen, Per Christian and Saxild-Hansen, Maria},
  journal={Journal of Computational and Applied Mathematics},
  volume={236},
  number={8},
  pages={2167--2178},
  year={2012},
  publisher={Elsevier}
}

@article{liang2018improving,
  title={Improving {FISTA}: Faster, Smarter and Greedier},
  author={Liang, Jingwei and Sch{\"o}nlieb, Carola-Bibiane},
  journal={arXiv preprint arXiv:1811.01430},
  year={2018}
}

@article{JanSochman2013,
  title={Implementation of TV denoising algorithms from "{A. Chambolle, T. Pock.} {A First-Order Primal-Dual Algorithm for Convex Problems with Applications to Imaging. Journal of Mathematical Imaging and Vision, 2011}"},
  author={Jan Sochman},
  journal={github.com/JanSochman/TVdenoising},
  year={2018}
}

@article{boyd2003subgradient,
  title={Subgradient methods},
  author={Boyd, Stephen and Xiao, Lin and Mutapcic, Almir},
  journal={lecture notes of EE392o, Stanford University, Autumn Quarter},
  volume={2004},
  pages={2004--2005},
  year={2003}
}


@article{yuan2006model,
  title={Model selection and estimation in regression with grouped variables},
  author={Yuan, Ming and Lin, Yi},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={68},
  number={1},
  pages={49--67},
  year={2006},
  publisher={Wiley Online Library}
}

@book{bauschke2011convex,
  title={Convex analysis and monotone operator theory in Hilbert spaces},
  author={Bauschke, Heinz H and Combettes, Patrick L and others},
  volume={408},
  year={2011},
  publisher={Springer}
}

@book{vapnik2013nature,
  title={The nature of statistical learning theory},
  author={Vapnik, Vladimir},
  year={2013},
  publisher={Springer science \& business media}
}

@article{wainwright2014structured,
  title={Structured regularizers for high-dimensional problems: Statistical and computational issues},
  author={Wainwright, Martin J},
  journal={Annual Review of Statistics and Its Application},
  volume={1},
  pages={233--253},
  year={2014},
  publisher={Annual Reviews}
}

@incollection{tsybakov2003optimal,
  title={Optimal rates of aggregation},
  author={Tsybakov, Alexandre B},
  booktitle={Learning Theory and Kernel Machines},
  pages={303--313},
  year={2003},
  publisher={Springer}
}

@article{pesquet2014class,
  title={A class of randomized primal-dual algorithms for distributed optimization},
  author={Pesquet, Jean-Christophe and Repetti, Audrey},
  journal={arXiv preprint arXiv:1406.6404},
  year={2014}
}

@article{sun2019online,
  title={An online plug-and-play algorithm for regularized image reconstruction},
  author={Sun, Yu and Wohlberg, Brendt and Kamilov, Ulugbek S},
  journal={IEEE Transactions on Computational Imaging},
  year={2019},
  publisher={IEEE}
}

@article{chin2018empirical,
  title={An Empirical Evaluation of Sketched SVD and its Application to Leverage Score Ordering},
  author={Chin, Hui Han and Liang, Paul Pu},
  journal={arXiv preprint arXiv:1812.07903},
  year={2018}
}

@inproceedings{dahiya2018empirical,
  title={An empirical evaluation of sketching for numerical linear algebra},
  author={Dahiya, Yogesh and Konomis, Dimitris and Woodruff, David P},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1292--1300},
  year={2018},
  organization={ACM}
}

@article{woodruff2014sketching,
  title={Sketching as a tool for numerical linear algebra},
  author={Woodruff, David P and others},
  journal={Foundations and Trends{\textregistered} in Theoretical Computer Science},
  volume={10},
  number={1--2},
  pages={1--157},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{dabov2007image,
  title={Image denoising by sparse 3-D transform-domain collaborative filtering.},
  author={Dabov, K and Foi, A and Katkovnik, V and Egiazarian, K},
  journal={IEEE transactions on image processing: a publication of the IEEE Signal Processing Society},
  volume={16},
  number={8},
  pages={2080--2095},
  year={2007}
}

@inproceedings{buades2005non,
  title={A non-local algorithm for image denoising},
  author={Buades, Antoni and Coll, Bartomeu and Morel, J-M},
  booktitle={2005 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'05)},
  volume={2},
  pages={60--65},
  year={2005},
  organization={IEEE}
}

@article{wang2006penalized,
  title={Penalized weighted least-squares approach to sinogram noise reduction and image reconstruction for low-dose X-ray computed tomography},
  author={Wang, Jing and Li, Tianfang and Lu, Hongbing and Liang, Zhengrong},
  journal={IEEE transactions on medical imaging},
  volume={25},
  number={10},
  pages={1272--1283},
  year={2006},
  publisher={IEEE}
}

@article{douglas1956numerical,
  title={On the numerical solution of heat conduction problems in two and three space variables},
  author={Douglas, Jim and Rachford, Henry H},
  journal={Transactions of the American mathematical Society},
  volume={82},
  number={2},
  pages={421--439},
  year={1956},
  publisher={JSTOR}
}

@article{boct2015inertial,
  title={Inertial Douglas--Rachford splitting for monotone inclusion problems},
  author={Bo{\c{t}}, Radu Ioan and Csetnek, Ern{\"o} Robert and Hendrich, Christopher},
  journal={Applied Mathematics and Computation},
  volume={256},
  pages={472--487},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{ulyanov2018deep,
  title={Deep image prior},
  author={Ulyanov, Dmitry and Vedaldi, Andrea and Lempitsky, Victor},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={9446--9454},
  year={2018}
}

@article{lehtinen2018noise2noise,
  title={Noise2noise: Learning image restoration without clean data},
  author={Lehtinen, Jaakko and Munkberg, Jacob and Hasselgren, Jon and Laine, Samuli and Karras, Tero and Aittala, Miika and Aila, Timo},
  journal={arXiv preprint arXiv:1803.04189},
  year={2018}
}

@article{sreehari2016plug,
  title={Plug-and-play priors for bright field electron tomography and sparse interpolation},
  author={Sreehari, Suhas and Venkatakrishnan, S Venkat and Wohlberg, Brendt and Buzzard, Gregery T and Drummy, Lawrence F and Simmons, Jeffrey P and Bouman, Charles A},
  journal={IEEE Transactions on Computational Imaging},
  volume={2},
  number={4},
  pages={408--423},
  year={2016},
  publisher={IEEE}
}

@article{talebi2013global,
  title={Global image denoising},
  author={Talebi, Hossein and Milanfar, Peyman},
  journal={IEEE Transactions on Image Processing},
  volume={23},
  number={2},
  pages={755--768},
  year={2013},
  publisher={IEEE}
}

@article{oymak2017sharp,
  title={Sharp time--data tradeoffs for linear inverse problems},
  author={Oymak, Samet and Recht, Benjamin and Soltanolkotabi, Mahdi},
  journal={IEEE Transactions on Information Theory},
  volume={64},
  number={6},
  pages={4129--4158},
  year={2017},
  publisher={IEEE}
}

@article{xu2020boosting,
  title={Boosting the Performance of Plug-and-Play Priors via Denoiser Scaling},
  author={Xu, Xiaojian and Liu, Jiaming and Sun, Yu and Wohlberg, Brendt and Kamilov, Ulugbek S},
  journal={arXiv preprint arXiv:2002.11546},
  year={2020}
}

@inproceedings{egiazarian2007compressed,
  title={Compressed sensing image reconstruction via recursive spatially adaptive filtering},
  author={Egiazarian, Karen and Foi, Alessandro and Katkovnik, Vladimir},
  booktitle={2007 IEEE International Conference on Image Processing},
  volume={1},
  pages={I--549},
  year={2007},
  organization={IEEE}
}

@inproceedings{needell2014stochastic,
  title={Stochastic gradient descent, weighted sampling, and the randomized kaczmarz algorithm},
  author={Needell, Deanna and Ward, Rachel and Srebro, Nati},
  booktitle={Advances in neural information processing systems},
  pages={1017--1025},
  year={2014}
}

@inproceedings{ryu2019plug,
  title={Plug-and-Play Methods Provably Converge with Properly Trained Denoisers},
  author={Ryu, Ernest and Liu, Jialin and Wang, Sicheng and Chen, Xiaohan and Wang, Zhangyang and Yin, Wotao},
  booktitle={International Conference on Machine Learning},
  pages={5546--5557},
  year={2019}
}

@article{gavaskar2020plug,
  title={Plug-and-play ISTA converges with kernel denoisers},
  author={Gavaskar, Ruturaj G and Chaudhury, Kunal N},
  journal={arXiv preprint arXiv:2004.03145},
  year={2020}
}

@article{chen2017trainable,
  title={Trainable nonlinear reaction diffusion: A flexible framework for fast and effective image restoration},
  author={Chen, Yunjin and Pock, Thomas},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={39},
  number={6},
  pages={1256--1272},
  year={2017},
  publisher={IEEE}
}

@article{zhang2017beyond,
  title={Beyond a gaussian denoiser: Residual learning of deep cnn for image denoising},
  author={Zhang, Kai and Zuo, Wangmeng and Chen, Yunjin and Meng, Deyu and Zhang, Lei},
  journal={IEEE Transactions on Image Processing},
  volume={26},
  number={7},
  pages={3142--3155},
  year={2017},
  publisher={IEEE}
}

@inproceedings{dabov2008image,
  title={Image restoration by sparse 3D transform-domain collaborative filtering},
  author={Dabov, Kostadin and Foi, Alessandro and Katkovnik, Vladimir and Egiazarian, Karen},
  booktitle={Image Processing: Algorithms and Systems VI},
  volume={6812},
  pages={681207},
  year={2008},
  organization={International Society for Optics and Photonics}
}


@article{bourgain2015toward,
  title={Toward a unified theory of sparse dimensionality reduction in euclidean space},
  author={Bourgain, Jean and Dirksen, Sjoerd and Nelson, Jelani},
  journal={Geometric and Functional Analysis},
  volume={25},
  number={4},
  pages={1009--1088},
  year={2015},
  publisher={Springer}
}

@article{lee2014proximal,
  title={Proximal Newton-type methods for minimizing composite functions},
  author={Lee, Jason D and Sun, Yuekai and Saunders, Michael A},
  journal={SIAM Journal on Optimization},
  volume={24},
  number={3},
  pages={1420--1443},
  year={2014},
  publisher={SIAM}
}


@inproceedings{cohen2018simple,
  title={Simple Analyses of the Sparse Johnson-Lindenstrauss Transform},
  author={Cohen, Michael B and Jayram, TS and Nelson, Jelani},
  booktitle={OASIcs-OpenAccess Series in Informatics},
  volume={61},
  year={2018},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@inproceedings{combettes2016stochastic,
  title={Stochastic forward-backward and primal-dual approximation algorithms with application to online image restoration},
  author={Combettes, Patrick L and Pesquet, Jean-Christophe},
  booktitle={Signal Processing Conference (EUSIPCO), 2016 24th European},
  pages={1813--1817},
  year={2016},
  organization={IEEE}
}

@inproceedings{zhu20041,
  title={1-norm support vector machines},
  author={Zhu, Ji and Rosset, Saharon and Tibshirani, Robert and Hastie, Trevor J},
  booktitle={Advances in neural information processing systems},
  pages={49--56},
  year={2004}
}

@inproceedings{scieur2016regularized,
  title={Regularized nonlinear acceleration},
  author={Scieur, Damien and d'Aspremont, Alexandre and Bach, Francis},
  booktitle={Advances In Neural Information Processing Systems},
  pages={712--720},
  year={2016}
}

@article{lin2016generic,
  title={A Generic Quasi-Newton Algorithm for Faster Gradient-Based Optimization},
  author={Lin, Hongzhou and Mairal, Julien and Harchaoui, Zaid},
  journal={arXiv preprint arXiv:1610.00960},
  year={2016}
}

@inproceedings{scieur2017nonlinear,
  title={Nonlinear acceleration of stochastic algorithms},
  author={Scieur, Damien and Bach, Francis and d'Aspremont, Alexandre},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3982--3991},
  year={2017}
}

@inproceedings{becker2012quasi,
  title={A quasi-Newton proximal splitting method},
  author={Becker, Stephen and Fadili, Jalal},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2618--2626},
  year={2012}
}

@article{chouzenoux2013majorize,
  title={A majorize-minimize subspace approach for $\backslash$ell\_2-$\backslash$ell\_0 image regularization},
  author={Chouzenoux, Emilie and Jezierska, Anna and Pesquet, Jean-Christophe and Talbot, Hugues},
  journal={SIAM Journal on Imaging Sciences},
  volume={6},
  number={1},
  pages={563--591},
  year={2013},
  publisher={SIAM}
}



@article{chouzenoux2014variable,
  title={Variable metric forward--backward algorithm for minimizing the sum of a differentiable function and a convex function},
  author={Chouzenoux, Emilie and Pesquet, Jean-Christophe and Repetti, Audrey},
  journal={Journal of Optimization Theory and Applications},
  volume={162},
  number={1},
  pages={107--132},
  year={2014},
  publisher={Springer}
}

@article{chouzenoux2016convergence,
  title={Convergence Rate Analysis of the Majorize-Minimize Subspace Algorithm},
  author={Chouzenoux, Emilie and Pesquet, Jean-Christophe},
  journal={IEEE Signal Processing Letters},
  volume={23},
  pages={1284--1288},
  year={2016}
}

@article{chouzenoux2016block,
  title={A block coordinate variable metric forward--backward algorithm},
  author={Chouzenoux, Emilie and Pesquet, Jean-Christophe and Repetti, Audrey},
  journal={Journal of Global Optimization},
  volume={66},
  number={3},
  pages={457--485},
  year={2016},
  publisher={Springer}
}

@article{friedman2004discussion,
  title={Discussion of “consistency in boosting”},
  author={Friedman, Jerome and Hastie, Trevor and Rosset, Saharon and Tibshirani, Robert and Zhu, Ji},
  journal={Annals of Statistics},
  volume={32},
  number={1},
  pages={102--107},
  year={2004}
}

@article{duchi2011adaptive,
  title={Adaptive subgradient methods for online learning and stochastic optimization},
  author={Duchi, John and Hazan, Elad and Singer, Yoram},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={Jul},
  pages={2121--2159},
  year={2011}
}



@inproceedings{allen2016optimal,
  title={Optimal black-box reductions between optimization objectives},
  author={Allen-Zhu, Zeyuan and Hazan, Elad},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1614--1622},
  year={2016}
}

@inproceedings{hu2009accelerated,
  title={Accelerated gradient methods for stochastic optimization and online learning},
  author={Hu, Chonghai and Pan, Weike and Kwok, James T},
  booktitle={Advances in Neural Information Processing Systems},
  pages={781--789},
  year={2009}
}

@inproceedings{amit2007uncovering,
  title={Uncovering shared structures in multiclass classification},
  author={Amit, Yonatan and Fink, Michael and Srebro, Nathan and Ullman, Shimon},
  booktitle={Proceedings of the 24th international conference on Machine learning},
  pages={17--24},
  year={2007},
  organization={ACM}
}

@article{moreau1961fonctions,
  title={Fonctions convexes duales et points proximaux dans un espace hilbertien},
  author={Moreau, Jean Jacques},
  journal={Comptes rendus hebdomadaires des s{\'e}ances de l'Acad{\'e}mie des sciences},
  volume={255},
  pages={2897--2899},
  year={1961}
}

@incollection{combettes2011proximal,
  title={Proximal splitting methods in signal processing},
  author={Combettes, Patrick L and Pesquet, Jean-Christophe},
  booktitle={Fixed-point algorithms for inverse problems in science and engineering},
  pages={185--212},
  year={2011},
  publisher={Springer}
}

@article{argyriou2008convex,
  title={Convex multi-task feature learning},
  author={Argyriou, Andreas and Evgeniou, Theodoros and Pontil, Massimiliano},
  journal={Machine Learning},
  volume={73},
  number={3},
  pages={243--272},
  year={2008},
  publisher={Springer}
}

@inproceedings{hu2009accelerated,
  title={Accelerated gradient methods for stochastic optimization and online learning},
  author={Hu, Chonghai and Pan, Weike and Kwok, James T},
  booktitle={Advances in Neural Information Processing Systems},
  pages={781--789},
  year={2009}
}

@article{allen2017katyusha,
  title={Katyusha: The first direct acceleration of stochastic gradient methods},
  author={Allen-Zhu, Zeyuan},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={8194--8244},
  year={2017},
  publisher={JMLR. org}
}

@article{yang2017weighted,
  title={Weighted SGD for ℓ p regression with randomized preconditioning},
  author={Yang, Jiyan and Chow, Yin-Lam and R{\'e}, Christopher and Mahoney, Michael W},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={7811--7853},
  year={2017},
  publisher={JMLR. org}
}

@article{tang2018structure,
  title={Structure-Adaptive Accelerated Coordinate Descent},
  author={Tang, Junqi and Golbabaee, Mohammad and Bach, Francis and Davies, Mike},
  year={2018},
  journal={Hal-archive hal-01889990v2}
}

@inproceedings{liang2014local,
  title={Local linear convergence of Forward--Backward under partial smoothness},
  author={Liang, Jingwei and Fadili, Jalal and Peyr{\'e}, Gabriel},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1970--1978},
  year={2014}
}

@article{liang2017local,
  title={Local convergence properties of douglas--rachford and alternating direction method of multipliers},
  author={Liang, Jingwei and Fadili, Jalal and Peyr{\'e}, Gabriel},
  journal={Journal of Optimization Theory and Applications},
  volume={172},
  number={3},
  pages={874--913},
  year={2017},
  publisher={Springer}
}

@article{liang2018local,
  title={Local linear convergence analysis of Primal--Dual splitting methods},
  author={Liang, Jingwei and Fadili, Jalal and Peyr{\'e}, Gabriel},
  journal={Optimization},
  volume={67},
  number={6},
  pages={821--853},
  year={2018},
  publisher={Taylor \& Francis}
}


@article{poon2018local,
  title={Local Convergence Properties of SAGA/Prox-SVRG and Acceleration},
  author={Poon, Clarice and Liang, Jingwei and Sch{\"o}nlieb, Carola-Bibiane},
  journal={arXiv preprint arXiv:1802.02554},
  year={2018}
}







@article{lin2015accelerated,
  title={An accelerated randomized proximal coordinate gradient method and its application to regularized empirical risk minimization},
  author={Lin, Qihang and Lu, Zhaosong and Xiao, Lin},
  journal={SIAM Journal on Optimization},
  volume={25},
  number={4},
  pages={2244--2273},
  year={2015},
  publisher={SIAM}
}

@inproceedings{allen2016even,
  title={Even faster accelerated coordinate descent using non-uniform sampling},
  author={Allen-Zhu, Zeyuan and Qu, Zheng and Richt{\'a}rik, Peter and Yuan, Yang},
  booktitle={International Conference on Machine Learning},
  pages={1110--1119},
  year={2016}
}

@article{wright2015coordinate,
  title={Coordinate descent algorithms},
  author={Wright, Stephen J},
  journal={Mathematical Programming},
  volume={151},
  number={1},
  pages={3--34},
  year={2015},
  publisher={Springer}
}

@article{chang2011libsvm,
  title={LIBSVM: a library for support vector machines},
  author={Chang, Chih-Chung and Lin, Chih-Jen},
  journal={ACM transactions on intelligent systems and technology (TIST)},
  volume={2},
  number={3},
  pages={27},
  year={2011},
  publisher={Acm}
}

@misc{REGED,
	author = "Causality workbench team",
	title = "A genomics dataset",
	year = "2008",
	month = "09",
	url = "http://www.causality.inf.ethz.ch/data/REGED.html",
	institution = "Causality workbench repository" }

@misc{MARTI,
	author = "Causality W-team",
	title = "Measurement Artifacts",
	year = "2008",
	month = "09",
	url = "http://www.causality.inf.ethz.ch/data/MARTI.html",
	institution = "Causality workbench repository" }






@InProceedings{pmlr-v80-lu18b,
  title = 	 {Accelerating Greedy Coordinate Descent Methods},
  author = 	 {Lu, Haihao and Freund, Robert and Mirrokni, Vahab},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {3257--3266},
  year = 	 {2018},
  volume = 	 {80},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {10--15 Jul},
  publisher = 	 {PMLR},
}

@inproceedings{lee2013efficient,
  title={Efficient Accelerated Coordinate Descent Methods and Faster Algorithms for Solving Linear Systems},
  author={Lee, Yin Tat and Sidford, Aaron},
  booktitle={Foundations of Computer Science (FOCS), 2013 IEEE 54th Annual Symposium on},
  pages={147--156},
  year={2013},
  organization={IEEE}
}

@article{csiba2016coordinate,
  title={Coordinate Descent Face-Off: Primal or Dual?},
  author={Csiba, Dominik and Richt{\'a}rik, Peter},
  journal={arXiv preprint arXiv:1605.08982},
  year={2016}
}


@inproceedings{lin2014adaptive,
  title={An adaptive accelerated proximal gradient method and its homotopy continuation for sparse optimization},
  author={Lin, Qihang and Xiao, Lin},
  booktitle={International Conference on Machine Learning},
  pages={73--81},
  year={2014}
}

@article{wen2017linear,
  title={Linear convergence of proximal gradient algorithm with extrapolation for a class of nonconvex nonsmooth minimization problems},
  author={Wen, Bo and Chen, Xiaojun and Pong, Ting Kei},
  journal={SIAM Journal on Optimization},
  volume={27},
  number={1},
  pages={124--145},
  year={2017},
  publisher={SIAM}
}

@book{buhlmann2011statistics,
  title={Statistics for high-dimensional data: methods, theory and applications},
  author={B{\"u}hlmann, Peter and Van De Geer, Sara},
  year={2011},
  publisher={Springer Science \& Business Media}
}

@book{van2000empirical,
  title={Empirical Processes in M-estimation},
  author={van de Geer, Sara},
  volume={6},
  year={2000},
  publisher={Cambridge university press}
}

@inproceedings{nutini2015coordinate,
  title={Coordinate descent converges faster with the Gauss-Southwell rule than random selection},
  author={Nutini, Julie and Schmidt, Mark and Laradji, Issam and Friedlander, Michael and Koepke, Hoyt},
  booktitle={International Conference on Machine Learning},
  pages={1632--1641},
  year={2015}
}


@article{lu2015complexity,
  title={On the complexity analysis of randomized block-coordinate descent methods},
  author={Lu, Zhaosong and Xiao, Lin},
  journal={Mathematical Programming},
  volume={152},
  number={1-2},
  pages={615--642},
  year={2015},
  publisher={Springer}
}
@article{bach2012optimization,
  title={Optimization with sparsity-inducing penalties},
  author={Bach, Francis and Jenatton, Rodolphe and Mairal, Julien and Obozinski, Guillaume and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={4},
  number={1},
  pages={1--106},
  year={2012},
  publisher={Now Publishers, Inc.}
}

@article{bickel2006regularization,
  title={Regularization in statistics},
  author={Bickel, Peter J and Li, Bo and Tsybakov, Alexandre B and van de Geer, Sara A and Yu, Bin and Vald{\'e}s, Te{\'o}filo and Rivero, Carlos and Fan, Jianqing and van der Vaart, Aad},
  journal={Test},
  volume={15},
  number={2},
  pages={271--344},
  year={2006},
  publisher={Springer}
}

@article{rennie2001improving,
  title={Improving multi-class text classification with naive Bayes},
  author={Rennie, Jason DM},
  year={2001}
}


@article{bach2008consistency,
  title={Consistency of the group lasso and multiple kernel learning},
  author={Bach, Francis R},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={Jun},
  pages={1179--1225},
  year={2008}
}

@article{vapnik1999overview,
  title={An overview of statistical learning theory},
  author={Vapnik, Vladimir Naumovich},
  journal={IEEE transactions on neural networks},
  volume={10},
  number={5},
  pages={988--999},
  year={1999},
  publisher={IEEE}
}

@article{candes2009exact,
  title={Exact matrix completion via convex optimization},
  author={Cand{\`e}s, Emmanuel J and Recht, Benjamin},
  journal={Foundations of Computational mathematics},
  volume={9},
  number={6},
  pages={717},
  year={2009},
  publisher={Springer}
}

@article{cai2010singular,
  title={A singular value thresholding algorithm for matrix completion},
  author={Cai, Jian-Feng and Cand{\`e}s, Emmanuel J and Shen, Zuowei},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={4},
  pages={1956--1982},
  year={2010},
  publisher={SIAM}
}

@book{tibshirani2015statistical,
  title={Statistical learning with sparsity: the lasso and generalizations},
  author={Tibshirani, Robert and Wainwright, Martin and Hastie, Trevor},
  year={2015},
  publisher={Chapman and Hall/CRC}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  pages={267--288},
  year={1996},
  publisher={JSTOR}
}

@article{tibshirani2005sparsity,
  title={Sparsity and smoothness via the fused lasso},
  author={Tibshirani, Robert and Saunders, Michael and Rosset, Saharon and Zhu, Ji and Knight, Keith},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={67},
  number={1},
  pages={91--108},
  year={2005},
  publisher={Wiley Online Library}
}



@article{allen2014linear,
	title={Linear coupling: An ultimate unification of gradient and mirror descent},
	author={Allen-Zhu, Zeyuan and Orecchia, Lorenzo},
	journal={arXiv preprint arXiv:1407.1537},
	year={2014}
}

@article{fercoq2018restarting,
  title={Restarting the accelerated coordinate descent method with a rough strong convexity estimate},
  author={Fercoq, Olivier and Qu, Zheng},
  journal={arXiv preprint arXiv:1803.05771},
  year={2018}
}

@inproceedings{murata2017doubly,
  title={Doubly accelerated stochastic variance reduced dual averaging method for regularized empirical risk minimization},
  author={Murata, Tomoya and Suzuki, Taiji},
  booktitle={Advances in Neural Information Processing Systems},
  pages={608--617},
  year={2017}
}

@inproceedings{zhang2004solving,
	title={Solving large scale linear prediction problems using stochastic gradient descent algorithms},
	author={Zhang, Tong},
	booktitle={Proceedings of the twenty-first international conference on Machine learning},
	pages={116},
	year={2004},
	organization={ACM}
}

@incollection{bottou2010large,
	title={Large-scale machine learning with stochastic gradient descent},
	author={Bottou, L{\'e}on},
	booktitle={Proceedings of COMPSTAT'2010},
	pages={177--186},
	year={2010},
	publisher={Springer}
}

@incollection{NIPS2014_5610,
	title = {Stochastic Proximal Gradient Descent with Acceleration Techniques},
	author = {Nitanda, Atsushi},
	booktitle = {Advances in Neural Information Processing Systems 27},
	editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
	pages = {1574--1582},
	year = {2014},
	publisher = {Curran Associates, Inc.},
	url = {http://papers.nips.cc/paper/5610-stochastic-proximal-gradient-descent-with-acceleration-techniques.pdf}
}

@article{raskutti2010restricted,
	title={Restricted eigenvalue properties for correlated Gaussian designs},
	author={Raskutti, Garvesh and Wainwright, Martin J and Yu, Bin},
	journal={Journal of Machine Learning Research},
	volume={11},
	number={Aug},
	pages={2241--2259},
	year={2010}
}

@article{shalev2013stochastic,
	title={Stochastic dual coordinate ascent methods for regularized loss minimization},
	author={Shalev-Shwartz, Shai and Zhang, Tong},
	journal={Journal of Machine Learning Research},
	volume={14},
	number={Feb},
	pages={567--599},
	year={2013}
}
@inproceedings{shalev2014accelerated,
	title={Accelerated proximal stochastic dual coordinate ascent for regularized loss minimization},
	author={Shalev-Shwartz, Shai and Zhang, Tong},
	booktitle={International Conference on Machine Learning},
	pages={64--72},
	year={2014}
}

@inproceedings{zhang2015stochastic,
	title={Stochastic primal-dual coordinate method for regularized empirical risk minimization},
	author={Zhang, Yuchen and Lin, Xiao},
	booktitle={Proceedings of the 32nd International Conference on Machine Learning (ICML-15)},
	pages={353--361},
	year={2015}
}

@article{lan2015optimal,
	title={An optimal randomized incremental gradient method},
	author={Lan, Guanghui and Zhou, Yi},
	journal={arXiv preprint arXiv:1507.02000},
	year={2015}
}

@inproceedings{karimi2016linear,
	title={Linear convergence of gradient and proximal-gradient methods under the polyak-{\l}ojasiewicz condition},
	author={Karimi, Hamed and Nutini, Julie and Schmidt, Mark},
	booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
	pages={795--811},
	year={2016},
	organization={Springer}
}

@inproceedings{roulet2017sharpness,
  title={Sharpness, restart and acceleration},
  author={Roulet, Vincent and d'Aspremont, Alexandre},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1119--1129},
  year={2017}
}

@article{qu2017linear,
	title={Linear convergence of SDCA in statistical estimation},
	author={Qu, Chao and Xu, Huan},
	journal={arXiv preprint arXiv:1701.07808},
	year={2017}
}

@article{nesterov2017efficiency,
  title={Efficiency of the accelerated coordinate descent method on structured optimization problems},
  author={Nesterov, Yurii and Stich, Sebastian U},
  journal={SIAM Journal on Optimization},
  volume={27},
  number={1},
  pages={110--123},
  year={2017},
  publisher={SIAM}
}

@inproceedings{arjevani2017limitations,
  title={Limitations on Variance-Reduction and Acceleration Schemes for Finite Sums Optimization},
  author={Arjevani, Yossi},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3543--3552},
  year={2017}
}




@book{nesterov2013introductory,
	title={Introductory lectures on convex optimization: A basic course},
	author={Nesterov, Yurii},
	volume={87},
	year={2013},
	publisher={Springer Science \& Business Media}
}
@inproceedings{nesterov1983method,
	title={A method of solving a convex programming problem with convergence rate O (1/k2)},
	author={Nesterov, Yurii},
	booktitle={Soviet Mathematics Doklady},
	volume={27},
	number={2},
	pages={372--376},
	year={1983}
}


@article{l2009sparse,
	title={Sparse online learning via truncated gradient},
	author={Langford, J. and Li, L. and Zhang, T.},
	journal={Journal of Machine Learning Research},
	volume={10},
	number={Mar},
	pages={777--801},
	year={2009}
}

@article{vaiter2015model,
  title={Model selection with low complexity priors},
  author={Vaiter, Samuel and Golbabaee, Mohammad and Fadili, Jalal and Peyr{\'e}, Gabriel},
  journal={Information and Inference: A Journal of the IMA},
  volume={4},
  number={3},
  pages={230--287},
  year={2015},
  publisher={Oxford University Press}
}
@article{tang2017structure,
	title={Structure-Adaptive, Variance-Reduced, and Accelerated Stochastic Optimization},
	author={Tang, Junqi and Bach, Francis and Golbabaee, Mohammad and Davies, Mike},
	journal={arXiv preprint arXiv:1712.03156},
	year={2017}
}

@article{pilanci2017newton,
	title={Newton sketch: A near linear-time optimization algorithm with linear-quadratic convergence},
	author={Pilanci, Mert and Wainwright, Martin J},
	journal={SIAM Journal on Optimization},
	volume={27},
	number={1},
	pages={205--245},
	year={2017},
	publisher={SIAM}
}
@article{negahban2012unified,
	title={A Unified Framework for High-Dimensional Analysis of M-Estimators with Decomposable Regularizers},
	author={Negahban, Sahand N and Ravikumar, Pradeep and Wainwright, Martin J and Yu, Bin},
	journal={Statistical Science},
	pages={538--557},
	year={2012},
	publisher={JSTOR}
}
@article{ndiaye2016gap,
	title={Gap Safe screening rules for sparsity enforcing penalties},
	author={Ndiaye, Eugene and Fercoq, Olivier and Gramfort, Alexandre and Salmon, Joseph},
	journal={arXiv preprint arXiv:1611.05780},
	year={2016}
}

@inproceedings{song2017accelerated,
	title={Accelerated Stochastic Greedy Coordinate Descent by Soft Thresholding Projection onto Simplex},
	author={Song, Chaobing and Cui, Shaobo and Jiang, Yong and Xia, Shu-Tao},
	booktitle={Advances in Neural Information Processing Systems},
	pages={4841--4850},
	year={2017}
}

@inproceedings{tang2017exploiting,
  title={Exploiting the structure via sketched gradient algorithms},
  author={Tang, Junqi and Golbabaee, Mohammad and Davies, Mike},
  booktitle={2017 IEEE Global Conference on Signal and Information Processing (GlobalSIP)},
  pages={1305--1309},
  year={2017},
  organization={IEEE}
}

@InProceedings{pmlr-v70-tang17a,
	title = 	 {Gradient Projection Iterative Sketch for Large-Scale Constrained Least-Squares},
	author = 	 {Junqi Tang and Mohammad Golbabaee and Mike E. Davies},
	booktitle = 	 {Proceedings of the 34th International Conference on Machine Learning},
	pages = 	 {3377--3386},
	year = 	 {2017},
	volume = 	 {70},
	series = 	 {Proceedings of Machine Learning Research},
	publisher = 	 {PMLR},
}
@incollection{defazio2016simple,
	title = {A Simple Practical Accelerated Method for Finite Sums},
	author = {Defazio, Aaron},
	booktitle = {Advances in Neural Information Processing Systems 29},
	editor = {D. D. Lee and M. Sugiyama and U. V. Luxburg and I. Guyon and R. Garnett},
	pages = {676--684},
	year = {2016},
	publisher = {Curran Associates, Inc.}
}

@article{bolte2007lojasiewicz,
  title={The {\L}ojasiewicz inequality for nonsmooth subanalytic functions with applications to subgradient dynamical systems},
  author={Bolte, J{\'e}r{\^o}me and Daniilidis, Aris and Lewis, Adrian},
  journal={SIAM Journal on Optimization},
  volume={17},
  number={4},
  pages={1205--1223},
  year={2007},
  publisher={SIAM}
}

@inproceedings{nitanda2014stochastic,
	title={Stochastic proximal gradient descent with acceleration techniques},
	author={Nitanda, Atsushi},
	booktitle={Advances in Neural Information Processing Systems},
	pages={1574--1582},
	year={2014}
}

@InProceedings{pmlr-v70-wang17l,
	title = 	 {Exploiting Strong Convexity from Data with Primal-Dual First-Order Algorithms},
	author = 	 {Jialei Wang and Lin Xiao},
	booktitle = 	 {Proceedings of the 34th International Conference on Machine Learning},
	pages = 	 {3694--3702},
	year = 	 {2017},
	editor = 	 {Doina Precup and Yee Whye Teh},
	volume = 	 {70},
	series = 	 {Proceedings of Machine Learning Research},
	address = 	 {International Convention Centre, Sydney, Australia},
	month = 	 {06--11 Aug},
	publisher = 	 {PMLR},
	pdf = 	 {http://proceedings.mlr.press/v70/wang17l/wang17l.pdf},
	url = 	 {http://proceedings.mlr.press/v70/wang17l.html},
	
}


@inproceedings{lin2014accelerated,
	title={An accelerated proximal coordinate gradient method},
	author={Lin, Qihang and Lu, Zhaosong and Xiao, Lin},
	booktitle={Advances in Neural Information Processing Systems},
	pages={3059--3067},
	year={2014}
}

@article{qu2016linear,
	title={Linear convergence of SVRG in statistical estimation},
	author={Qu, Chao and Xu, Huan},
	journal={arXiv preprint arXiv:1611.01957},
	year={2016}
}

@article{qu2017saga,
	title={SAGA and Restricted Strong Convexity},
	author={Qu, Chao and Li, Yan and Xu, Huan},
	journal={arXiv preprint arXiv:1702.05683},
	year={2017}
}

@misc{Lichman:2013 ,
	author = "M. Lichman",
	year = "2013",
	title = "{UCI} Machine Learning Repository",
	url = "http://archive.ics.uci.edu/ml",
	institution = "University of California, Irvine, School of Information and Computer Sciences" }



@article{chandrasekaran2013computational,
	title={Computational and statistical tradeoffs via convex relaxation},
	author={Chandrasekaran, V. and Jordan, M. I.},
	journal={Proceedings of the National Academy of Sciences},
	volume={110},
	number={13},
	pages={E1181--E1190},
	year={2013},
	publisher={National Acad Sciences}
}

@inproceedings{shalev2016sdca,
  title={Sdca without duality, regularization, and individual convexity},
  author={Shalev-Shwartz, Shai},
  booktitle={International Conference on Machine Learning},
  pages={747--754},
  year={2016}
}

@inproceedings{allen2016katyusha,
  title={Katyusha: The first direct acceleration of stochastic gradient methods},
  author={Allen-Zhu, Zeyuan},
  booktitle={Proceedings of the 49th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={1200--1205},
  year={2017},
  organization={ACM}
}

@misc{van2007spgl1,
	title={SPGL1: A solver for large-scale sparse reconstruction},
	author={Van Den Berg, E. and Friedlander, M. P.},
	year={2007},
	publisher={June}
}

@article{johnson1984extensions,
	title={Extensions of Lipschitz mappings into a Hilbert space},
	author={Johnson, W. B. and Lindenstrauss, J.},
	journal={Contemporary mathematics},
	volume={26},
	number={189-206},
	pages={1},
	year={1984}
}

@article{dasgupta2003elementary,
	title={An elementary proof of a theorem of Johnson and Lindenstrauss},
	author={Dasgupta, S. and Gupta, A.},
	journal={Random Structures \& Algorithms},
	volume={22},
	number={1},
	pages={60--65},
	year={2003},
	publisher={Wiley Online Library}
}

@article{chambolle2018stochastic,
  title={Stochastic primal-dual hybrid gradient algorithm with arbitrary sampling and imaging applications},
  author={Chambolle, Antonin and Ehrhardt, Matthias J and Richtarik, Peter and Schonlieb, Carola-Bibiane},
  journal={SIAM Journal on Optimization},
  volume={28},
  number={4},
  pages={2783--2808},
  year={2018},
  publisher={SIAM}
}

@article{kapralov2016fake,
	title={How to Fake Multiply by a Gaussian Matrix},
	author={Kapralov, M. and Potluru, V. K. and Woodruff, D. P.},
	journal={arXiv preprint arXiv:1606.05732},
	year={2016}
}

@article{wang2015practical,
	title={A Practical Guide to Randomized Matrix Computations with MATLAB Implementations},
	author={Wang, S.},
	journal={arXiv preprint arXiv:1505.07570},
	year={2015}
}

@article{shalev2011stochastic,
	title={Stochastic methods for l1-regularized loss minimization},
	author={Shalev-Shwartz, S. and Tewari, A.},
	journal={Journal of Machine Learning Research},
	volume={12},
	number={Jun},
	pages={1865--1892},
	year={2011}
}

@article{konevcny2016mini,
	title={Mini-batch semi-stochastic gradient descent in the proximal setting},
	author={Kone{\v{c}}n{\`y}, Jakub and Liu, Jie and Richt{\'a}rik, Peter and Tak{\'a}{\v{c}}, Martin},
	journal={IEEE Journal of Selected Topics in Signal Processing},
	volume={10},
	number={2},
	pages={242--255},
	year={2016},
	publisher={IEEE}
}


@article{schmidt2013minimizing,
	title={Minimizing finite sums with the stochastic average gradient},
	author={Schmidt, M. and Le Roux, N. and Bach, F.},
	journal={Mathematical Programming},
	pages={1--30},
	year={2013},
	publisher={Springer}
}

@inproceedings{clarkson2013low,
	title={Low rank approximation and regression in input sparsity time},
	author={Clarkson, K. L. and Woodruff, D. P.},
	booktitle={Proceedings of the forty-fifth annual ACM symposium on Theory of computing},
	pages={81--90},
	year={2013},
	organization={ACM}
}


@article{agarwal2012fast,
	author={Agarwal, A. and Negahban, S. and Wainwright, M. J.},	
	title={Fast global convergence rates of gradient methods for high-dimensional statistical recovery},

	journal={The Annals of Statistics},
	volume={40},
	number={5},
	pages={2452--2482},
	year={2012}
}
@inproceedings{lin2015universal,
	title={A universal catalyst for first-order optimization},
	author={Lin, H. and Mairal, J. and Harchaoui, Z.},
	booktitle={Advances in Neural Information Processing Systems},
	pages={3384--3392},
	year={2015}
}

@article{giryes2016tradeoffs,
	title={Tradeoffs between Convergence Speed and Reconstruction Accuracy in Inverse Problems},
	author={Giryes, R. and Eldar, Y. C. and Bronstein, A. M. and Sapiro, G.},
	journal={arXiv preprint arXiv:1605.09232},
	year={2016}
}




@article{blumensath2011sampling,
	title={Sampling and reconstructing signals from a union of linear subspaces},
	author={Blumensath, T.},
	journal={IEEE Transactions on Information Theory},
	volume={57},
	number={7},
	pages={4660--4671},
	year={2011},
	publisher={IEEE}
}



@article{o2015adaptive,
	title={Adaptive restart for accelerated gradient schemes},
	author={O'Donoghue, B. and Candes, E.},
	journal={Foundations of computational mathematics},
	volume={15},
	number={3},
	pages={715--732},
	year={2015},
	publisher={Springer}
}
@article{baraniuk2008simple,
	title={A simple proof of the restricted isometry property for random matrices},
	author={Baraniuk, R. and Davenport, M. and DeVore, R. and Wakin, M.},
	journal={Constructive Approximation},
	volume={28},
	number={3},
	pages={253--263},
	year={2008},
	publisher={Springer}
}

@techreport{nesterov2007gradient,
	title={Gradient methods for minimizing composite objective function},
	author={Nesterov, Y.},
	year={2007},
	institution={UCL}
}

@article{nesterov2013gradient,
	title={Gradient methods for minimizing composite functions},
	author={Nesterov, Y.},
	journal={Mathematical Programming},
	volume={140},
	number={1},
	pages={125--161},
	year={2013},
	publisher={Springer}
}

@article{xiao2014proximal,
	title={A proximal stochastic gradient method with progressive variance reduction},
	author={Xiao, L. and Zhang, T.},
	journal={SIAM Journal on Optimization},
	volume={24},
	number={4},
	pages={2057--2075},
	year={2014},
	publisher={SIAM}
}

@article{candes2006stable,
	title={Stable signal recovery from incomplete and inaccurate measurements},
	author={Candes, E. and Romberg, J. and Tao, T.},
	journal={Communications on pure and applied mathematics},
	volume={59},
	number={8},
	pages={1207--1223},
	year={2006},
	publisher={Wiley Online Library}
}

@article{drineas2011faster,
	title={Faster least squares approximation},
	author={Drineas, P. and Mahoney, M. W. and Muthukrishnan, S. and Sarl{\'o}s, T.},
	journal={Numerische Mathematik},
	volume={117},
	number={2},
	pages={219--249},
	year={2011},
	publisher={Springer}
}

@article{beck2009fast,
	title={Fast gradient-based algorithms for constrained total variation image denoising and deblurring problems},
	author={Beck, A. and Teboulle, M.},
	journal={IEEE Transactions on Image Processing},
	volume={18},
	number={11},
	pages={2419--2434},
	year={2009},
	publisher={IEEE}
}

@article{mahoney2011randomized,
	title={Randomized algorithms for matrices and data},
	author={Mahoney, M. W.},
	journal={Foundations and Trends{\textregistered} in Machine Learning},
	volume={3},
	number={2},
	pages={123--224},
	year={2011},
	publisher={Now Publishers Inc.}
}






@article{candes2008restricted,
	title={The restricted isometry property and its implications for compressed sensing},
	author={Candes, E. J.},
	journal={Comptes Rendus Mathematique},
	volume={346},
	number={9},
	pages={589--592},
	year={2008},
	publisher={Elsevier}
}

@article{2016_Pilanci_Iterative,
	title={Iterative Hessian Sketch: Fast and Accurate Solution Approximation for Constrained Least-Squares},
	author={Pilanci, M. and Wainwright, M. J.},
	journal={Journal of Machine Learning Research},
	volume={17},
	number={53},
	pages={1--38},
	year={2016}
}

@ARTICLE{Figueiredo2007gradient, 
	author={M. A. T. Figueiredo and R. D. Nowak and S. J. Wright}, 
	journal={IEEE Journal of Selected Topics in Signal Processing}, 
	title={Gradient Projection for Sparse Reconstruction: Application to Compressed Sensing and Other Inverse Problems}, 
	year={2007}, 
	volume={1}, 
	number={4}, 
	pages={586-597}, 
	ISSN={1932-4553}, 
	month={Dec},}



@article{hazan2016variance,
	title={Variance-reduced and projection-free stochastic optimization},
	author={Hazan, E. and Luo, H.},
	journal={arXiv preprint arXiv:1602.02101},
	year={2016}
}





@inproceedings{jaggi2013revisiting,
	title={Revisiting Frank-Wolfe: Projection-Free Sparse Convex Optimization.},
	author={Jaggi, M.},
	booktitle={ICML (1)},
	pages={427--435},
	year={2013}
}

@inproceedings{shamir2013stochastic,
	title={Stochastic Gradient Descent for Non-smooth Optimization: Convergence Results and Optimal Averaging Schemes.},
	author={Shamir, Ohad and Zhang, Tong},
	booktitle={ICML (1)},
	pages={71--79},
	year={2013}
}



@inproceedings{defazio2014saga,
	title={SAGA: A fast incremental gradient method with support for non-strongly convex composite objectives},
	author={Defazio, A. and Bach, F. and Lacoste-Julien, S.},
	booktitle={Advances in Neural Information Processing Systems},
	pages={1646--1654},
	year={2014}
}

@article{gong2014linear,
	title={Linear Convergence of Variance-Reduced Stochastic Gradient without Strong Convexity},
	author={Gong, Pinghua and Ye, Jieping},
	journal={arXiv preprint arXiv:1406.1102},
	year={2014}
}

@article{nguyen2014linear,
	title={Linear convergence of stochastic iterative greedy algorithms with sparse constraints},
	author={Nguyen, Nam and Needell, Deanna and Woolf, Tina},
	journal={arXiv preprint arXiv:1407.0088},
	year={2014}
}

@article{li2016stochastic,
	title={Stochastic Variance Reduced Optimization for Nonconvex Sparse Learning},
	author={Li, X. and Zhao, T. and Arora, R. and Liu, H. and Haupt, J.},
	journal={arXiv preprint arXiv:1605.02711},
	year={2016}
}

@article{shen2016tight,
	title={A Tight Bound of Hard Thresholding},
	author={Shen, J. and Li, P.},
	journal={arXiv preprint arXiv:1605.01656},
	year={2016}
}

@inproceedings{woodworth2016tight,
  title={Tight complexity bounds for optimizing composite objectives},
  author={Woodworth, Blake E and Srebro, Nati},
  booktitle={Advances in neural information processing systems},
  pages={3639--3647},
  year={2016}
}

@article{fercoq2017adaptive,
	title={Adaptive restart of accelerated gradient methods under local quadratic growth condition},
	author={Fercoq, Olivier and Qu, Zheng},
	journal={arXiv preprint arXiv:1709.02300},
	year={2017}
}

@inproceedings{agarwal2010fast,
	title={Fast global convergence rates of gradient methods for high-dimensional statistical recovery},
	author={Agarwal, A. and Negahban, S. and Wainwright, M. J.},
	booktitle={Advances in Neural Information Processing Systems},
	pages={37--45},
	year={2010}
}

@inproceedings{2014_Needell_Stochastic,
	title={Stochastic gradient descent, weighted sampling, and the randomized kaczmarz algorithm},
	author={Needell, Deanna and Ward, Rachel and Srebro, Nati},
	booktitle={Advances in Neural Information Processing Systems},
	pages={1017--1025},
	year={2014}
}

@inproceedings{2011_Moulines_Non,
	title={Non-asymptotic analysis of stochastic approximation algorithms for machine learning},
	author={Moulines, Eric and Bach, Francis R},
	booktitle={Advances in Neural Information Processing Systems},
	pages={451--459},
	year={2011}
}

@article{2010_Rudelson_Nonasymptotic,
	title={Non-asymptotic theory of random matrices: extreme singular values},
	author={Rudelson, Mark and Vershynin, Roman},
	journal={arXiv preprint arXiv:1003.2990},
	year={2010}
}


@article{2015_Oymak_Universality,
	title={Universality laws for randomized dimension reduction, with applications},
	author={Oymak, S. and Tropp, J. A.},
	journal={arXiv preprint arXiv:1511.09433},
	year={2015}
}

@article{2008_Gilbert_Tutorial,
	title={A tutorial on fast fourier sampling},
	author={Gilbert, Anna C and Strauss, Martin J and Tropp, Joel A},
	journal={Signal processing magazine, IEEE},
	volume={25},
	number={2},
	pages={57--66},
	year={2008},
	publisher={IEEE}
}

@article{2014_Gilbert_Recent,
	title={Recent developments in the sparse fourier transform: a compressed fourier transform for big data},
	author={Gilbert, Anna C and Indyk, Piotr and Iwen, Mark and Schmidt, Ludwig},
	journal={Signal Processing Magazine, IEEE},
	volume={31},
	number={5},
	pages={91--100},
	year={2014},
	publisher={IEEE}
}

@article{fercoq2016restarting,
	title={Restarting accelerated gradient methods with a rough strong convexity estimate},
	author={Fercoq, Olivier and Qu, Zheng},
	journal={arXiv preprint arXiv:1609.07358},
	year={2016}
}

@article{2005_Cormode_Improved,
	title={An improved data stream summary: the count-min sketch and its applications},
	author={Cormode, Graham and Muthukrishnan, S},
	journal={Journal of Algorithms},
	volume={55},
	number={1},
	pages={58--75},
	year={2005},
	publisher={Elsevier}
}

@article{2016_Daniely_Sketching,
	title={Sketching and Neural Networks},
	author={Daniely, Amit and Lazic, Nevena and Singer, Yoram and Talwar, Kunal},
	journal={arXiv preprint arXiv:1604.05753},
	year={2016}
}

@article{2012_Chandrasekaran_Convex,
	title={The convex geometry of linear inverse problems},
	author={Chandrasekaran, V. and Recht, B. and Parrilo, P. A. and Willsky, A. S.},
	journal={Foundations of Computational mathematics},
	volume={12},
	number={6},
	pages={805--849},
	year={2012},
	publisher={Springer}
}

@inproceedings{2015_Li_Sublinear,
	title={Sub-linear time compressed sensing using sparse-graph codes},
	author={Li, Xiao and Pawar, Sameer and Ramchandran, Kannan},
	booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
	pages={1645--1649},
	year={2015},
	organization={IEEE}
}

@article{2011_Halko_Finding,
	title={Finding structure with randomness: Probabilistic algorithms for constructing approximate matrix decompositions},
	author={Halko, Nathan and Martinsson, Per-Gunnar and Tropp, Joel A},
	journal={SIAM review},
	volume={53},
	number={2},
	pages={217--288},
	year={2011},
	publisher={SIAM}
}


@article{2005_Combettes_Signal,
	title={Signal recovery by proximal forward-backward splitting},
	author={Combettes, Patrick L and Wajs, Val{\'e}rie R},
	journal={Multiscale Modeling \& Simulation},
	volume={4},
	number={4},
	pages={1168--1200},
	year={2005},
	publisher={SIAM}
}

@incollection{2011_Combettes_Proximal,
	title={Proximal splitting methods in signal processing},
	author={Combettes, P. L. and Pesquet, J.},
	booktitle={Fixed-point algorithms for inverse problems in science and engineering},
	pages={185--212},
	year={2011},
	publisher={Springer}
}

@article{2013_Xiang_Regularization,
	title={Regularization with randomized SVD for large-scale discrete inverse problems},
	author={Xiang, Hua and Zou, Jun},
	journal={Inverse Problems},
	volume={29},
	number={8},
	pages={085008},
	year={2013},
	publisher={IOP Publishing}
}


@Article{1984_Johnson_Extensions,
	author="Johnson, William B.
	and Lindenstrauss, Joram
	and Schechtman, Gideon",
	title="Extensions of lipschitz maps into Banach spaces",
	journal="Israel Journal of Mathematics",
	year="1986",
	volume="54",
	number="2",
	pages="129--138",
	abstract="It is proved that ifY ⊂X are metric spaces withY havingn≧2 points then any mapf fromY into a Banach spaceZ can be extended to a map                                                                          \$\${\backslash}hat f\$\$                 fromX intoZ so that                                                                          \$\${\backslash}left{\backslash}| \{{\backslash}hat f\} {\backslash}right{\backslash}|\_\{lip\}  {\backslash}leqq c log n{\backslash}left{\backslash}| f {\backslash}right{\backslash}|\_\{lip\} \$\$                 wherec is an absolute constant. A related result is obtained for the case whereX is assumed to be a finite-dimensional normed space andY is an arbitrary subset ofX.",
	issn="1565-8511",
	doi="10.1007/BF02764938",
	url="http://dx.doi.org/10.1007/BF02764938"
}



@Article{2008_Ailon_Fast,
	author="Ailon, N.
	and Liberty, E.",
	title="Fast Dimension Reduction Using Rademacher Series on Dual BCH Codes",
	journal="Discrete \& Computational Geometry",
	year="2008",
	volume="42",
	number="4",
	pages="615--630"
}



@article{2009_Ailon_Fast,
	author = {N. Ailon and B. Chazelle},
	title = {The Fast Johnson–Lindenstrauss Transform and Approximate Nearest Neighbors},
	journal = {SIAM Journal on Computing},
	volume = {39},
	number = {1},
	pages = {302-322},
	year = {2009}
	
}





@INCOLLECTION{2012_Roux_Stochastic,
	author = {Nicolas L. Roux and Schmidt, Mark and Francis R. Bach},
	title = {A Stochastic Gradient Method with an Exponential Convergence \_Rate
	for Finite Training Sets},
	booktitle = {Advances in Neural Information Processing Systems 25},
	publisher = {Curran Associates, Inc.},
	year = {2012},
	editor = {F. Pereira and C. J. C. Burges and L. Bottou and K. Q. Weinberger},
	pages = {2663--2671}
}

@ARTICLE{2007_Bioucas_TwIST,
	author={J. M. Bioucas-Dias and M. A. T. Figueiredo},
	journal={IEEE Transactions on Image Processing},
	title={A New TwIST: Two-Step Iterative Shrinkage/Thresholding Algorithms for Image Restoration},
	year={2007},
	volume={16},
	number={12},
	pages={2992-3004},
	keywords={convergence;image restoration;image segmentation;inverse problems;iterative methods;optimisation;wavelet transforms;TwIST algorithm;convex unconstrained optimization problem;image restoration;image segmentation;image thresholding algorithm;iterative shrinkage;linear inverse problem;linear observation model;nonquadratic regularizer;Convex analysis;image deconvolution;image restoration;non-smooth optimization;optimization;regularization;total variation;wavelets;Algorithms;Image Enhancement;Image Interpretation, Computer-Assisted;Pattern Recognition, Automated;Reproducibility of Results;Sensitivity and Specificity;Signal Processing, Computer-Assisted},
	doi={10.1109/TIP.2007.909319},
	ISSN={1057-7149},
	month={Dec},}

@incollection{2013_Johnson_Accelerating,
	title = {Accelerating Stochastic Gradient Descent using Predictive Variance Reduction},
	author = {Johnson, R. and Zhang, T.},
	booktitle = {Advances in Neural Information Processing Systems 26},
	pages = {315--323},
	year = {2013},
	publisher = {Curran Associates, Inc.},
	
}


@article{2014_Pilanci_Iterative,
	author =       "M. Pilanci and M. Wainwright.",
	title =        "{Iterative Hessian sketch: Fast and accurate solution approximation for constrained least-squares}",
	journal =      "arXiv:1411.0347",
	month   =      "Nov.",
	year =         "2014"
}

@ARTICLE{2008_Candes_Introduction,
	author={Candes, E. J. and Wakin, M. B.},
	journal={Signal Processing Magazine, IEEE},
	title={An Introduction To Compressive Sampling},
	year={2008},
	volume={25},
	number={2},
	pages={21-30},
	doi={10.1109/MSP.2007.914731},
	ISSN={1053-5888},
	month={March},}

@ARTICLE{2015_Davenport_Constrained,
	author = {{Davenport}, M.~A. and {Massimino}, A.~K. and {Needell}, D. and 
	{Woolf}, T.},
	title = "{Constrained adaptive sensing}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1506.05889},
	primaryClass = "cs.IT",
	keywords = {Computer Science - Information Theory},
	year = 2015,
	month = jun,
	adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150605889D},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013_Arias_Fundamental,
	author={Arias-Castro, E. and Candes, E. J. and Davenport, M. A.},
	journal={Information Theory, IEEE Transactions on},
	title={On the Fundamental Limits of Adaptive Sensing},
	year={2013},
	volume={59},
	number={1},
	pages={472-481},
	doi={10.1109/TIT.2012.2215837},
	ISSN={0018-9448},
	month={Jan},}



@article{2008_Roklin_Fast,
	author = {Rokhlin, V. and Tygert, M.}, 
	title = {A fast randomized algorithm for overdetermined linear least-squares regression},
	volume = {105}, 
	number = {36}, 
	pages = {13212-13217}, 
	year = {2008}, 
	doi = {10.1073/pnas.0804869105},  
	URL = {http://www.pnas.org/content/105/36/13212.abstract}, 
	eprint = {http://www.pnas.org/content/105/36/13212.full.pdf}, 
	journal = {Proceedings of the National Academy of Sciences} 
}

@article{2010_Avron_Blendenpik,
	author = {H. Avron and P. Maymounkov and Sivan Toledo},
	title = {Blendenpik: Supercharging LAPACK's Least-Squares Solver},
	journal = {SIAM Journal on Scientific Computing},
	volume = {32},
	number = {3},
	pages = {1217-1236},
	year = {2010},
	doi = {10.1137/090767911},
	
	URL = { 
	http://dx.doi.org/10.1137/090767911
	
	},
	eprint = { 
	http://dx.doi.org/10.1137/090767911
	
	}
}

@article{2013_Chandrasekaran_Computational,
	author = {Chandrasekaran, V. and Jordan, M. I.}, 
	title = {Computational and statistical tradeoffs via convex relaxation},
	volume = {110}, 
	number = {13}, 
	pages = {E1181-E1190}, 
	year = {2013}, 
	doi = {10.1073/pnas.1302293110}, 
	URL = {http://www.pnas.org/content/110/13/E1181.abstract}, 
	eprint = {http://www.pnas.org/content/110/13/E1181.full.pdf}, 
	journal = {Proceedings of the National Academy of Sciences} 
}

@ARTICLE{2015_Yang_Weighted,
	author = {{Yang}, J. and {Chow}, Y.-L. and {R{\'e}}, C. and {Mahoney}, M.~W.
	},
	title = "{Weighted SGD for $\ell\_p$ Regression with Randomized Preconditioning}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1502.03571},
	primaryClass = "math.OC",
	year = 2015,
	month = feb,
	adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150203571Y},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@book{2004_Boyed_Convex,
	title={Convex optimization},
	author={Boyd, Stephen and Vandenberghe, Lieven},
	year={2004},
	publisher={Cambridge university press}
}

@article{2014_Kane_Sparser,
	author = {Kane, Daniel M. and Nelson, Jelani},
	title = {Sparser Johnson-Lindenstrauss Transforms},
	journal = {J. ACM},
	issue_date = {January 2014},
	volume = {61},
	number = {1},
	month = jan,
	year = {2014},
	issn = {0004-5411},
	pages = {4:1--4:23},
	articleno = {4},
	numpages = {23},
	url = {http://doi.acm.org/10.1145/2559902},
	doi = {10.1145/2559902},
	acmid = {2559902},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Dimensionality reduction, Johnson-Lindenstrauss, numerical linear algebra, streaming algorithms},
} 

@inproceedings{perelli2019regularized,
  title={Regularized Newton Sketch by Denoising Score Matching for Computed Tomography Reconstruction},
  author={Perelli, Alessandro and Andersen, Martin Skovgaard},
  booktitle={2019 Workshop on Signal Processing with Adaptive Sparse Structured Representations},
  year={2019}
}

@article{mai2019anderson,
  title={Anderson Acceleration of Proximal Gradient Methods},
  author={Mai, Vien V and Johansson, Mikael},
  journal={arXiv preprint arXiv:1910.08590},
  year={2019}
}

@article{1999_Erdogan_Ordered,
	author={H Erdogan and J A Fessler},
	title={Ordered subsets algorithms for transmission tomography},
	journal={Physics in Medicine and Biology},
	volume={44},
	number={11},
	pages={2835},
	url={http://stacks.iop.org/0031-9155/44/i=11/a=311},
	year={1999},
}2015_Oymak_Sharp

@article{2015_Oymak_Sharp,
	title={Sharp Time--Data Tradeoffs for Linear Inverse Problems},
	author={Oymak, S. and Recht, B. and Soltanolkotabi, M.},
	journal={arXiv preprint arXiv:1507.04793},
	year={2015}
}

@article{2009_Beck_Fast,
	author = {A. Beck and M. Teboulle},
	title = {A Fast Iterative Shrinkage-Thresholding Algorithm for Linear Inverse Problems},
	journal = {SIAM Journal on Imaging Sciences},
	volume = {2},
	number = {1},
	pages = {183-202},
	year = {2009}
}



@ARTICLE{2014_Goldstein_Field,
	author = {{Goldstein}, T. and {Studer}, C. and {Baraniuk}, R.},
	title = "{A Field Guide to Forward-Backward Splitting with a FASTA Implementation}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1411.3406},
	primaryClass = "cs.NA",
	keywords = {Computer Science - Numerical Analysis, G.1.6},
	year = 2014,
	month = nov,
	adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1411.3406G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{2011_Becker_Fast,
	author = {Stephen Becker and Jérôme Bobin and Emmanuel J. Candès},
	title = {NESTA: A Fast and Accurate First-Order Method for Sparse Recovery},
	journal = {SIAM Journal on Imaging Sciences},
	volume = {4},
	number = {1},
	pages = {1-39},
	year = {2011},
	doi = {10.1137/090756855},
	
	URL = { 
	http://dx.doi.org/10.1137/090756855
	
	},
	eprint = { 
	http://dx.doi.org/10.1137/090756855
	
	}
	
}





@article{2012_Drineas_Fast,
	author = {Drineas, Petros and Magdon-Ismail, Malik and Mahoney, Michael W. and Woodruff, David P.},
	title = {Fast Approximation of Matrix Coherence and Statistical Leverage},
	journal = {J. Mach. Learn. Res.},
	issue_date = {January 2012},
	volume = {13},
	number = {1},
	month = dec,
	year = {2012},
	issn = {1532-4435},
	pages = {3475--3506},
	numpages = {32},
	url = {http://dl.acm.org/citation.cfm?id=2503308.2503352},
	acmid = {2503352},
	publisher = {JMLR.org},
	keywords = {matrix coherence, randomized algorithm, statistical leverage},
} 


@article{2008_Blumensath_Iterative,
	title={Iterative thresholding for sparse approximations},
	author={Blumensath, Thomas and Davies, Mike E},
	journal={Journal of Fourier Analysis and Applications},
	volume={14},
	number={5-6},
	pages={629--654},
	year={2008},
	publisher={Springer}
}

@article{2013_Mairal_Stochastic,
	title={Stochastic majorization-minimization algorithms for large-scale optimization},
	author={Mairal, Julien},
	booktitle={Advances in Neural Information Processing Systems},
	pages={2283--2291},
	year={2013}
}


@article{2015_Pilanci_Randomized,
	title={Randomized sketches of convex programs with sharp guarantees},
	author={Pilanci, M. and Wainwright, M. J.},
	journal={Information Theory, IEEE Transactions on},
	volume={61},
	number={9},
	pages={5096--5115},
	year={2015},
	publisher={IEEE}
}
@inproceedings{johnson2013accelerating,
	title={Accelerating stochastic gradient descent using predictive variance reduction},
	author={Johnson, Rie and Zhang, Tong},
	booktitle={Advances in neural information processing systems},
	pages={315--323},
	year={2013}
}

@article{2015_Pilanci_Newton,
	title={Newton Sketch: A Linear-time Optimization Algorithm with Linear-Quadratic Convergence},
	author={Pilanci, Mert and Wainwright, Martin J},
	journal={arXiv preprint arXiv:1505.02250},
	year={2015}
}



@article{2013_Konecny_Semi-stochastic,
	title={Semi-stochastic gradient descent methods},
	author={Kone{\v{c}}n{\`y}, J. and Richt{\'a}rik, P.},
	journal={arXiv preprint arXiv:1312.1666},
	year={2013}
}

@ARTICLE{2015_Gower_Randomized,
	author = {{Gower}, R.~M. and {Richt{\'a}rik}, P.},
	title = "{Randomized Iterative Methods for Linear Systems}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1506.03296},
	primaryClass = "math.NA",
	keywords = {Mathematics - Numerical Analysis, 15A06, 15B52, 65F10, 68W20, 65N75, 65Y20, 68Q25, 68W40, 90C20, G.1.3},
	year = 2015,
	month = jun,
	adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150603296G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016_Gower_Stochastic,
	author = {{Gower}, R.~M. and {Goldfarb}, D. and {Richt{\'a}rik}, P.},
	title = "{Stochastic Block BFGS: Squeezing More Curvature out of Data}",
	journal = {ArXiv e-prints},
	archivePrefix = "arXiv",
	eprint = {1603.09649},
	primaryClass = "math.OC",
	keywords = {Mathematics - Optimization and Control, 90C53, 74S60, 90C06, 62L20, 68W20, 15B52, 65Y20, 68W40, G.1.6},
	year = 2016,
	month = mar,
	adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160309649G},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{2015_Oymak_Isometric,
	author    = {Samet Oymak and
	Benjamin Recht and
	Mahdi Soltanolkotabi},
	title     = {Isometric sketching of any set via the Restricted Isometry Property},
	journal   = {CoRR},
	volume    = {abs/1506.03521},
	year      = {2015},
	url       = {http://arxiv.org/abs/1506.03521},
	timestamp = {Wed, 01 Jul 2015 15:10:24 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/OymakRS15},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{2001_Achlioptas_Database,
	title = "Database-friendly random projections: Johnson-Lindenstrauss with binary coins ",
	journal = "Journal of Computer and System Sciences ",
	volume = "66",
	number = "4",
	pages = "671 - 687",
	year = "2003",
	note = "Special Issue on \{PODS\} 2001 ",
	issn = "0022-0000",
	doi = "http://dx.doi.org/10.1016/S0022-0000(03)00025-4",
	url = "http://www.sciencedirect.com/science/article/pii/S0022000003000254",
	author = "Dimitris Achlioptas",
	
}

@misc{2010_Nelson_Johnson,
	title={Johnson--Lindenstrauss notes},
	author={Nelson, Jelani},
	year = "2010",
	publisher={Citeseer}
}


@inproceedings{2010_Dasgupta_Sparse,
	title={A sparse johnson: Lindenstrauss transform},
	author={Dasgupta, Anirban and Kumar, Ravi and Sarl{\'o}s, Tam{\'a}s},
	booktitle={Proceedings of the forty-second ACM symposium on Theory of computing},
	pages={341--350},
	year={2010},
	organization={ACM}
}


@article{nesterov2012efficiency,
  title={Efficiency of coordinate descent methods on huge-scale optimization problems},
  author={Nesterov, Yu},
  journal={SIAM Journal on Optimization},
  volume={22},
  number={2},
  pages={341--362},
  year={2012},
  publisher={SIAM}
}

@article{fercoq2015accelerated,
  title={Accelerated, parallel, and proximal coordinate descent},
  author={Fercoq, Olivier and Richt{\'a}rik, Peter},
  journal={SIAM Journal on Optimization},
  volume={25},
  number={4},
  pages={1997--2023},
  year={2015},
  publisher={SIAM}
}


@article{wu2008coordinate,
  title={Coordinate descent algorithms for lasso penalized regression},
  author={Wu, Tong Tong and Lange, Kenneth and others},
  journal={The Annals of Applied Statistics},
  volume={2},
  number={1},
  pages={224--244},
  year={2008},
  publisher={Institute of Mathematical Statistics}
}

@incollection{wen2012block,
  title={Block coordinate descent methods for semidefinite programming},
  author={Wen, Zaiwen and Goldfarb, Donald and Scheinberg, Katya},
  booktitle={Handbook on Semidefinite, Conic and Polynomial Optimization},
  pages={533--564},
  year={2012},
  publisher={Springer}
}

@inproceedings{hsieh2008dual,
  title={A dual coordinate descent method for large-scale linear SVM},
  author={Hsieh, Cho-Jui and Chang, Kai-Wei and Lin, Chih-Jen and Keerthi, S Sathiya and Sundararajan, Sellamanickam},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={408--415},
  year={2008},
  organization={ACM}
}

@article{qin2013efficient,
  title={Efficient block-coordinate descent algorithms for the group lasso},
  author={Qin, Zhiwei and Scheinberg, Katya and Goldfarb, Donald},
  journal={Mathematical Programming Computation},
  volume={5},
  number={2},
  pages={143--169},
  year={2013},
  publisher={Springer}
}

@article{richtarik2014iteration,
  title={Iteration complexity of randomized block-coordinate descent methods for minimizing a composite function},
  author={Richt{\'a}rik, Peter and Tak{\'a}{\v{c}}, Martin},
  journal={Mathematical Programming},
  volume={144},
  number={1-2},
  pages={1--38},
  year={2014},
  publisher={Springer}
}



@article{2006_Donoho_Compressed,
	title={Compressed sensing},
	author={Donoho, D. L.},
	journal={Information Theory, IEEE Transactions on},
	volume={52},
	number={4},
	pages={1289--1306},
	year={2006},
	publisher={IEEE}
}

@book{vempala2005random,
  title={The random projection method},
  author={Vempala, Santosh S},
  volume={65},
  year={2005},
  publisher={American Mathematical Soc.}
}


@inproceedings{carratino2018learning,
  title={Learning with sgd and random features},
  author={Carratino, Luigi and Rudi, Alessandro and Rosasco, Lorenzo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={10212--10223},
  year={2018}
}

@inproceedings{rudi2015less,
  title={Less is more: Nystr{\"o}m computational regularization},
  author={Rudi, Alessandro and Camoriano, Raffaello and Rosasco, Lorenzo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1657--1665},
  year={2015}
}


@article{whyte2012non,
  title={Non-uniform deblurring for shaken images},
  author={Whyte, Oliver and Sivic, Josef and Zisserman, Andrew and Ponce, Jean},
  journal={International journal of computer vision},
  volume={98},
  number={2},
  pages={168--186},
  year={2012},
  publisher={Springer}
}

@article{raguet2013generalized,
  title={A generalized forward-backward splitting},
  author={Raguet, Hugo and Fadili, Jalal and Peyr{\'e}, Gabriel},
  journal={SIAM Journal on Imaging Sciences},
  volume={6},
  number={3},
  pages={1199--1226},
  year={2013},
  publisher={SIAM}
}




@inproceedings{shen2017gsos,
  title={GSOS: Gauss-Seidel Operator Splitting Algorithm for Multi-Term Nonsmooth Convex Composite Optimization},
  author={Shen, Li and Liu, Wei and Yuan, Ganzhao and Ma, Shiqian},
  booktitle={International Conference on Machine Learning},
  pages={3125--3134},
  year={2017}
}

@inproceedings{zhao2018stochastic,
  title={Stochastic Three-Composite Convex Minimization with a Linear Operator},
  author={Zhao, Renbo and Cevher, Volkan},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={765--774},
  year={2018}
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan and others},
  journal={Foundations and Trends{\textregistered} in Machine learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers, Inc.}
}



@article{nesterov2005smooth,
  title={Smooth minimization of non-smooth functions},
  author={Nesterov, Yu},
  journal={Mathematical programming},
  volume={103},
  number={1},
  pages={127--152},
  year={2005},
  publisher={Springer}
}

@inproceedings{alacaoglu2017smooth,
  title={Smooth Primal-Dual Coordinate Descent Algorithms for Nonsmooth Convex Optimization},
  author={Alacaoglu, Ahmet and Dinh, Quoc Tran and Fercoq, Olivier and Cevher, Volkan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5854--5863},
  year={2017}
}

@inproceedings{palaniappan2016stochastic,
  title={Stochastic variance reduction methods for saddle-point problems},
  author={Palaniappan, Balamurugan and Bach, Francis},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1416--1424},
  year={2016}
}

@InCollection{tang2018rest,
  Title                    = {Rest-Katyusha: Exploiting the Solution\textquotesingle s Structure via Scheduled Restart Schemes},
  Author                   = {Tang, Junqi and Golbabaee, Mohammad and Bach, Francis and davies, Mike E},
  Booktitle                = {Advances in Neural Information Processing Systems 31},
  Publisher                = {Curran Associates, Inc.},
  Year                     = {2018},
  Pages                    = {427--438}
}


@incollection{robbins1985stochastic,
  title={A stochastic approximation method},
  author={Robbins, Herbert and Monro, Sutton},
  booktitle={Herbert Robbins Selected Papers},
  pages={102--109},
  year={1985},
  publisher={Springer}
}

@article{karimi2017sparse,
  title={Sparse-View Image Reconstruction in Cone-Beam Computed Tomography with Variance-Reduced Stochastic Gradient Descent and Locally-Adaptive Proximal Operation},
  author={Karimi, Davood and Ward, Rabab K},
  journal={Journal of Medical and Biological Engineering},
  volume={37},
  number={3},
  pages={420--440},
  year={2017},
  publisher={Springer}
}

@online{kodim,
  author = {Kodak-Lossless-True-Color-Image-Suite},
  url = {http://r0k.us/graphics/kodak/}
}




@inproceedings{shen2017gsos,
  title={GSOS: Gauss-Seidel Operator Splitting Algorithm for Multi-Term Nonsmooth Convex Composite Optimization},
  author={Shen, Li and Liu, Wei and Yuan, Ganzhao and Ma, Shiqian},
  booktitle={International Conference on Machine Learning},
  pages={3125--3134},
  year={2017}
}






@article{allen2018katyusha,
  title={Katyusha X: Practical Momentum Method for Stochastic Sum-of-Nonconvex Optimization},
  author={Allen-Zhu, Zeyuan},
  journal={arXiv preprint arXiv:1802.03866},
  year={2018}
}



@inproceedings{ouyang2013stochastic,
  title={Stochastic alternating direction method of multipliers},
  author={Ouyang, Hua and He, Niao and Tran, Long and Gray, Alexander},
  booktitle={International Conference on Machine Learning},
  pages={80--88},
  year={2013}
}

@inproceedings{zhong2014accelerated,
  title={Accelerated stochastic gradient method for composite regularization},
  author={Zhong, Wenliang and Kwok, James},
  booktitle={Artificial Intelligence and Statistics},
  pages={1086--1094},
  year={2014}
}

@inproceedings{ehrhardt2017faster,
  title={Faster PET reconstruction with a stochastic primal-dual hybrid gradient method},
  author={Ehrhardt, Matthias J and Markiewicz, Pawel and Chambolle, Antonin and Richt{\'a}rik, Peter and Schott, Jonathan and Sch{\"o}nlieb, Carola-Bibiane},
  booktitle={Wavelets and Sparsity XVII},
  volume={10394},
  pages={103941O},
  year={2017},
  organization={International Society for Optics and Photonics}
}

@article{lan2012optimal,
  title={An optimal method for stochastic composite optimization},
  author={Lan, Guanghui},
  journal={Mathematical Programming},
  volume={133},
  number={1-2},
  pages={365--397},
  year={2012},
  publisher={Springer}
}

@article{karimi2016hybrid,
  title={A hybrid stochastic-deterministic gradient descent algorithm for image reconstruction in cone-beam computed tomography},
  author={Karimi, Davood and Ward, Rabab K},
  journal={Biomedical Physics \& Engineering Express},
  volume={2},
  number={1},
  pages={015008},
  year={2016},
  publisher={IOP Publishing}
}


@article{du2018linear,
  title={Linear Convergence of the Primal-Dual Gradient Method for Convex-Concave Saddle Point Problems without Strong Convexity},
  author={Du, Simon S and Hu, Wei},
  journal={arXiv preprint arXiv:1802.01504},
  year={2018}
}

@article{almeida2013deconvolving,
  title={Deconvolving images with unknown boundaries using the alternating direction method of multipliers},
  author={Almeida, Mariana SC and Figueiredo, Mario},
  journal={IEEE Transactions on Image processing},
  volume={22},
  number={8},
  pages={3074--3086},
  year={2013},
  publisher={IEEE}
}

@article{afonso2010fast,
  title={Fast image recovery using variable splitting and constrained optimization},
  author={Afonso, Manya V and Bioucas-Dias, Jos{\'e} M and Figueiredo, M{\'a}rio AT},
  journal={IEEE transactions on image processing},
  volume={19},
  number={9},
  pages={2345--2356},
  year={2010},
  publisher={IEEE}
}



@article{chambolle2011first,
  title={A first-order primal-dual algorithm for convex problems with applications to imaging},
  author={Chambolle, Antonin and Pock, Thomas},
  journal={Journal of mathematical imaging and vision},
  volume={40},
  number={1},
  pages={120--145},
  year={2011},
  publisher={Springer}
}

@article{chambolle2016ergodic,
  title={On the ergodic convergence rates of a first-order primal--dual algorithm},
  author={Chambolle, Antonin and Pock, Thomas},
  journal={Mathematical Programming},
  volume={159},
  number={1-2},
  pages={253--287},
  year={2016},
  publisher={Springer}
}


@inproceedings{allen2016improved,
  title={Improved SVRG for non-strongly-convex or sum-of-non-convex objectives},
  author={Allen-Zhu, Zeyuan and Yuan, Yang},
  booktitle={International conference on machine learning},
  pages={1080--1089},
  year={2016}
}


@article{erdogan1999ordered,
  title={Ordered subsets algorithms for transmission tomography},
  author={Erdogan, Hakan and Fessler, Jeffrey A},
  journal={Physics in Medicine \& Biology},
  volume={44},
  number={11},
  pages={2835},
  year={1999},
  publisher={IOP Publishing}
}

@article{kim2015combining,
  title={Combining ordered subsets and momentum for accelerated X-ray CT image reconstruction},
  author={Kim, Donghwan and Ramani, Sathish and Fessler, Jeffrey A},
  journal={IEEE transactions on medical imaging},
  volume={34},
  number={1},
  pages={167--178},
  year={2015},
  publisher={IEEE}
}


@inproceedings{almeida2013blind,
  title={Blind image deblurring with unknown boundaries using the alternating direction method of multipliers},
  author={Almeida, Mariana SC and Figueiredo, M{\'a}rio AT},
  booktitle={Image Processing (ICIP), 2013 20th IEEE International Conference on},
  pages={586--590},
  year={2013},
  organization={IEEE}
}



@article{zhao2015scalable,
  title={Scalable stochastic alternating direction method of multipliers},
  author={Zhao, Shen-Yi and Li, Wu-Jun and Zhou, Zhi-Hua},
  journal={arXiv preprint arXiv:1502.03529},
  year={2015}
}



@article{yang2017randomized,
  title={Randomized sketches for kernels: Fast and optimal nonparametric regression},
  author={Yang, Yun and Pilanci, Mert and Wainwright, Martin J and others},
  journal={The Annals of Statistics},
  volume={45},
  number={3},
  pages={991--1023},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{gonen2016solving,
  title={Solving ridge regression using sketched preconditioned svrg},
  author={Gonen, Alon and Orabona, Francesco and Shalev-Shwartz, Shai},
  booktitle={International Conference on Machine Learning},
  pages={1397--1405},
  year={2016}
}

@article{robbins1951stochastic,
  title={A Stochastic Approximation Method},
  author={Robbins, Herbert and Monro, Sutton},
  journal={The Annals of Mathematical Statistics},
  volume={22},
  number={3},
  pages={400--407},
  year={1951}
}

@article{danielyan2011bm3d,
  title={BM3D frames and variational image deblurring},
  author={Danielyan, Aram and Katkovnik, Vladimir and Egiazarian, Karen},
  journal={IEEE Transactions on Image Processing},
  volume={21},
  number={4},
  pages={1715--1728},
  year={2011},
  publisher={IEEE}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={Proceedings
of 3rd International Conference on Learning Representations},
  year={2015}
}

@article{lions1979splitting,
  title={Splitting algorithms for the sum of two nonlinear operators},
  author={Lions, Pierre-Louis and Mercier, Bertrand},
  journal={SIAM Journal on Numerical Analysis},
  volume={16},
  number={6},
  pages={964--979},
  year={1979},
  publisher={SIAM}
}

@article{lan2016gradient,
  title={Gradient sliding for composite optimization},
  author={Lan, Guanghui},
  journal={Mathematical Programming},
  volume={159},
  number={1-2},
  pages={201--235},
  year={2016},
  publisher={Springer}
}

@article{lan2016accelerated,
  title={Accelerated gradient sliding for structured convex optimization},
  author={Lan, Guanghui and Ouyang, Yuyuan},
  journal={arXiv preprint arXiv:1609.04905},
  year={2016}
}
@article{reddi2018convergence,
  title={On the convergence of adam and beyond},
  author={Reddi, Sashank J and Kale, Satyen and Kumar, Sanjiv},
  year={2018}
}

@article{luo2019adaptive,
  title={Adaptive gradient methods with dynamic bound of learning rate},
  author={Luo, Liangchen and Xiong, Yuanhao and Liu, Yan and Sun, Xu},
  journal={arXiv preprint arXiv:1902.09843},
  year={2019}
}

@article{perraudin2014unlocbox,
  title={UNLocBoX: A MATLAB convex optimization toolbox for proximal-splitting methods},
  author={Perraudin, Nathanael and Kalofolias, Vassilis and Shuman, David and Vandergheynst, Pierre},
  journal={arXiv preprint arXiv:1402.0779},
  year={2014}
}

@article{bredies2010total,
  title={Total generalized variation},
  author={Bredies, Kristian and Kunisch, Karl and Pock, Thomas},
  journal={SIAM Journal on Imaging Sciences},
  volume={3},
  number={3},
  pages={492--526},
  year={2010},
  publisher={SIAM}
}

@article{rudin1992nonlinear,
  title={Nonlinear total variation based noise removal algorithms},
  author={Rudin, Leonid I and Osher, Stanley and Fatemi, Emad},
  journal={Physica D: nonlinear phenomena},
  volume={60},
  number={1-4},
  pages={259--268},
  year={1992},
  publisher={Elsevier}
}

@inproceedings{agarwal2009information,
  title={Information-theoretic lower bounds on the oracle complexity of convex optimization},
  author={Agarwal, Alekh and Wainwright, Martin J and Bartlett, Peter L and Ravikumar, Pradeep K},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1--9},
  year={2009}
}

@article{mahoney2011randomized,
  title={Randomized algorithms for matrices and data},
  author={Mahoney, Michael W and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={3},
  number={2},
  pages={123--224},
  year={2011},
  publisher={Now Publishers, Inc.}
}

@article{tropp2017practical,
  title={Practical sketching algorithms for low-rank matrix approximation},
  author={Tropp, Joel A and Yurtsever, Alp and Udell, Madeleine and Cevher, Volkan},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={38},
  number={4},
  pages={1454--1485},
  year={2017},
  publisher={SIAM}
}

@inproceedings{cohen2015dimensionality,
  title={Dimensionality reduction for k-means clustering and low rank approximation},
  author={Cohen, Michael B and Elder, Sam and Musco, Cameron and Musco, Christopher and Persu, Madalina},
  booktitle={Proceedings of the forty-seventh annual ACM symposium on Theory of computing},
  pages={163--172},
  year={2015},
  organization={ACM}
}

@article{nikolova2004variational,
  title={A variational approach to remove outliers and impulse noise},
  author={Nikolova, Mila},
  journal={Journal of Mathematical Imaging and Vision},
  volume={20},
  number={1-2},
  pages={99--120},
  year={2004},
  publisher={Springer}
}

@incollection{tsybakov2003optimal,
  title={Optimal rates of aggregation},
  author={Tsybakov, Alexandre B},
  booktitle={Learning Theory and Kernel Machines},
  pages={303--313},
  year={2003},
  publisher={Springer}
}

@article{bubeck2015convex,
  title={Convex optimization: Algorithms and complexity},
  author={Bubeck, S{\'e}bastien},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={8},
  number={3-4},
  pages={231--357},
  year={2015},
  publisher={Now Publishers, Inc.}
}

@inproceedings{zhou2018simple,
  title={A Simple Stochastic Variance Reduced Algorithm with Fast Convergence Rates},
  author={Zhou, Kaiwen and Shang, Fanhua and Cheng, James},
  booktitle={International Conference on Machine Learning},
  pages={5975--5984},
  year={2018}
}

@inproceedings{allen2018lingering,
  title={The Lingering of Gradients: How to Reuse Gradients Over Time},
  author={Allen-Zhu, Zeyuan and Simchi-Levi, David and Wang, Xinshang},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1252--1261},
  year={2018}
}

@article{basu2000n,
  title={O$(N^2 \log_2 N)$ filtered backprojection reconstruction algorithm for tomography},
  author={Basu, Samit and Bresler, Yoram},
  journal={IEEE Transactions on Image Processing},
  volume={9},
  number={10},
  pages={1760--1773},
  year={2000},
  publisher={IEEE}
}

@article{lan2016conditional,
  title={Conditional gradient sliding for convex optimization},
  author={Lan, Guanghui and Zhou, Yi},
  journal={SIAM Journal on Optimization},
  volume={26},
  number={2},
  pages={1379--1409},
  year={2016},
  publisher={SIAM}
}

@book{rockafellar2015convex,
  title={Convex analysis},
  author={Rockafellar, Ralph Tyrell},
  year={2015},
  publisher={Princeton university press}
}

@article{moreau1965proximite,
  title={Proximit{\'e} et dualit{\'e} dans un espace hilbertien},
  author={Moreau, Jean-Jacques},
  journal={Bulletin de la Soci{\'e}t{\'e} math{\'e}matique de France},
  volume={93},
  pages={273--299},
  year={1965}
}

@article{zhou2018direct,
  title={Direct Acceleration of SAGA using Sampled Negative Momentum},
  author={Zhou, Kaiwen},
  journal={arXiv preprint arXiv:1806.11048},
  year={2018}
}

@inproceedings{mahdavi2013mixed,
  title={Mixed optimization for smooth functions},
  author={Mahdavi, Mehrdad and Zhang, Lijun and Jin, Rong},
  booktitle={Advances in Neural Information Processing Systems},
  pages={674--682},
  year={2013}
}

@inproceedings{tang2019limitation,
  title={The Limitation and Practical Acceleration of Stochastic Gradient Algorithms in Inverse Problems},
  author={Tang, Junqi and Egiazarian, Karen and Davies, Mike},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7680--7684},
  year={2019},
  organization={IEEE}
}

@article{2008_Candes_restricted,
	title = "The restricted isometry property and its implications for compressed sensing ",
	journal = "Comptes Rendus Mathematique ",
	volume = "346",
	number = "9–10",
	pages = "589 - 592",
	year = "2008",
	note = "",
	issn = "1631-073X",
	doi = "http://dx.doi.org/10.1016/j.crma.2008.03.014",
	url = "http://www.sciencedirect.com/science/article/pii/S1631073X08000964",
	author = "Emmanuel J. Candès"
}

@article{csiba2018importance,
  title={Importance sampling for minibatches},
  author={Csiba, Dominik and Richt{\'a}rik, Peter},
  journal={The Journal of Machine Learning Research},
  volume={19},
  number={1},
  pages={962--982},
  year={2018},
  publisher={JMLR. org}
}

@inproceedings{andoni2015practical,
  title={Practical and optimal LSH for angular distance},
  author={Andoni, Alexandr and Indyk, Piotr and Laarhoven, Thijs and Razenshteyn, Ilya and Schmidt, Ludwig},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1225--1233},
  year={2015}
}

@inproceedings{allen2016exploiting,
  title={Exploiting the structure: Stochastic gradient methods using raw clusters},
  author={Allen-Zhu, Zeyuan and Yuan, Yang and Sridharan, Karthik},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1642--1650},
  year={2016}
}

@inproceedings{hofmann2015variance,
  title={Variance reduced stochastic gradient descent with neighbors},
  author={Hofmann, Thomas and Lucchi, Aurelien and Lacoste-Julien, Simon and McWilliams, Brian},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2305--2313},
  year={2015}
}

@article{lee2016tracy,
  title={Tracy--Widom distribution for the largest eigenvalue of real sample covariance matrices with general population},
  author={Lee, Ji Oon and Schnelli, Kevin and others},
  journal={The Annals of Applied Probability},
  volume={26},
  number={6},
  pages={3786--3839},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{2014_Nelson_New,
	title={New constructions of RIP matrices with fast multiplication and fewer rows},
	author={Nelson, Jelani and Price, Eric and Wootters, Mary},
	booktitle={Proceedings of the Twenty-Fifth Annual ACM-SIAM Symposium on Discrete Algorithms},
	pages={1515--1528},
	year={2014},
	organization={SIAM}
}

@article{ono2017primal,
  title={Primal-dual plug-and-play image restoration},
  author={Ono, Shunsuke},
  journal={IEEE Signal Processing Letters},
  volume={24},
  number={8},
  pages={1108--1112},
  year={2017},
  publisher={IEEE}
}

@phdthesis{renbo2018stochastic,
  title={Stochastic and Randomized Algorithms for Large-Scale Optimization in Machine Learning},
  author={Renbo, Zhao},
  year={2018}
}



@article{chan2017plug,
  title={Plug-and-play ADMM for image restoration: Fixed-point convergence and applications},
  author={Chan, Stanley H and Wang, Xiran and Elgendy, Omar A},
  journal={IEEE Transactions on Computational Imaging},
  volume={3},
  number={1},
  pages={84--98},
  year={2017},
  publisher={IEEE}
}


@book{1988_Gordon_Milman,
	title={On Milman's inequality and random subspaces which escape through a mesh in $\mathcal{R}^n$},
	author={Gordon, Yehoram},
	year={1988},
	publisher={Springer}
}


@article{2011_Mahoney_Randomized,
	title={Randomized algorithms for matrices and data},
	author={Mahoney, M. W.},
	journal={Foundations and Trends{\textregistered} in Machine Learning},
	volume={3},
	number={2},
	pages={123--224},
	year={2011},
	publisher={Now Publishers Inc.}
}


@article{2005_Candes_Decoding,
	title={Decoding by linear programming},
	author={Candes, Emmanuel J and Tao, Terence},
	journal={Information Theory, IEEE Transactions on},
	volume={51},
	number={12},
	pages={4203--4215},
	year={2005},
	publisher={IEEE}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@Article{KoMa14,
  title =	 {An Adaptive Shifted Power Method for Computing
                  Generalized Tensor Eigenpairs},
  author =	 {Tamara G. Kolda and Jackson R. Mayo},
  doi =		 {10.1137/140951758},
  journal =	 {SIAM Journal on Matrix Analysis and Applications},
  number =	 4,
  volume =	 35,
  year =	 2014,
  month =	 dec,
  pages =	 {1563--1581},
}

@Misc{siam,
  key = {zzz},
  title =	 {{SIAM} Style Manual: For journals and books},
  year =	 2013,
url = {https://www.siam.org/journals/pdf/stylemanual.pdf}}

@Misc{Hi14,
  author =	 {Nick Higham},
  title =	 {A Call for Better Indexes},
  howpublished = {SIAM Blogs},
  year =	 2014,
  month =	 nov,
  url =		 {http://blogs.siam.org/a-call-for-better-indexes/},
  urldate =	 {2015-04-05}
}

@Misc{PeKoPi14,
  title = {Accelerating Community Detection by Using {K}-core Subgraphs},
  author =	 {Chengbin Peng and Tamara G. Kolda and Ali Pinar},
  eprint =	 {1403.2226},
  year =	 2014,
  month =	 mar,
  eprintclass =	 {math.NA}
}


@Article{WoZhMeSh05,
  author =	 {Woessner, Donald E. and Zhang, Shanrong and
                  Merritt, Matthew E. and Sherry, A. Dean},
  title = {Numerical Solution of the {Bloch} Equations Provides Insights 
                  into the Optimum Design of {PARACEST} Agents for {MRI}},
  journal =	 {Magnetic Resonance in Medicine},
  doi =		 {10.1002/mrm.20408},
  volume =	 53,
  number =	 4,
  month =	 apr,
  year =	 2005,
  pages =	 {790--799},
  archiveprefix = {PubMed},
  archive =	 {https://www.ncbi.nlm.nih.gov/pubmed},
  eprint =	 {15799055}
}
@article{lee2019solving2,
  title={Solving Linear Programs with Sqrt (rank) Linear System Solves},
  author={Lee, Yin Tat and Sidford, Aaron},
  journal={arXiv preprint arXiv:1910.08033},
  year={2019}
}

@inproceedings{adil2019iterative,
  title={Iterative Refinement for ℓp-norm Regression},
  author={Adil, Deeksha and Kyng, Rasmus and Peng, Richard and Sachdeva, Sushant},
  booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={1405--1424},
  year={2019},
  organization={SIAM}
}

@article{kerenidis2019quantum,
  title={Quantum algorithms for Second-Order Cone Programming and Support Vector Machines},
  author={Kerenidis, Iordanis and Prakash, Anupam and Szil{\'a}gyi, D{\'a}niel},
  journal={arXiv preprint arXiv:1908.06720},
  year={2019}
}

@inproceedings{cohen2019solving,
  title={Solving linear programs in the current matrix multiplication time},
  author={Cohen, Michael B and Lee, Yin Tat and Song, Zhao},
  booktitle={Proceedings of the 51st Annual ACM SIGACT Symposium on Theory of Computing},
  pages={938--942},
  year={2019},
  organization={ACM}
}

@article{lee2019solving,
  title={Solving Empirical Risk Minimization in the Current Matrix Multiplication Time},
  author={Lee, Yin Tat and Song, Zhao and Zhang, Qiuyi},
  journal={arXiv preprint arXiv:1905.04447},
  year={2019}
}

@inproceedings{shi2019sublinear,
  title={Sublinear Time Numerical Linear Algebra for Structured Matrices},
  author={Shi, Xiaofei and Woodruff, David P},
  booktitle={Proceedings of the AAAI},
  year={2019}
}

@inproceedings{avron2013sketching,
  title={Sketching structured matrices for faster nonlinear regression},
  author={Avron, Haim and Sindhwani, Vikas and Woodruff, David},
  booktitle={Advances in neural information processing systems},
  pages={2994--3002},
  year={2013}
}

@article{berahas2017investigation,
  title={An investigation of Newton-sketch and subsampled Newton methods},
  author={Berahas, Albert S and Bollapragada, Raghu and Nocedal, Jorge},
  journal={arXiv preprint arXiv:1705.06211},
  year={2017}
}

@inproceedings{rudi2017falkon,
  title={Falkon: An optimal large scale kernel method},
  author={Rudi, Alessandro and Carratino, Luigi and Rosasco, Lorenzo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3888--3898},
  year={2017}
}

@article{tang2019practicality,
  title={The Practicality of Stochastic Optimization in Imaging Inverse Problems},
  author={Tang, Junqi and Egiazarian, Karen and Golbabaee, Mohammad and Davies, Mike},
  journal={arXiv preprint arXiv:1910.10100},
  year={2019}
}

@article{poon2019trajectory,
  title={Trajectory of Alternating Direction Method of Multipliers and Adaptive Acceleration},
  author={Poon, Clarice and Liang, Jingwei},
  journal={arXiv preprint arXiv:1906.10114},
  year={2019}
}
@article{milanfar2012tour,
  title={A tour of modern image filtering: New insights and methods, both practical and theoretical},
  author={Milanfar, Peyman},
  journal={IEEE signal processing magazine},
  volume={30},
  number={1},
  pages={106--128},
  year={2012},
  publisher={IEEE}
}

@inproceedings{gidel2019implicit,
  title={Implicit regularization of discrete gradient dynamics in linear neural networks},
  author={Gidel, Gauthier and Bach, Francis and Lacoste-Julien, Simon},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3202--3211},
  year={2019}
}

@inproceedings{vaksman2020lidia,
  title={LIDIA: Lightweight Learned Image Denoising with Instance Adaptation},
  author={Vaksman, Gregory and Elad, Michael and Milanfar, Peyman},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={524--525},
  year={2020}
}

@article{mohammadnia2018convolutional,
  title={Convolutional kernel networks based on a convex combination of cosine kernels},
  author={Mohammadnia-Qaraei, Mohammad Reza and Monsefi, Reza and Ghiasi-Shirazi, Kamaledin},
  journal={Pattern Recognition Letters},
  volume={116},
  pages={127--134},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{mairal2014convolutional,
  title={Convolutional kernel networks},
  author={Mairal, Julien and Koniusz, Piotr and Harchaoui, Zaid and Schmid, Cordelia},
  booktitle={Advances in neural information processing systems},
  pages={2627--2635},
  year={2014}
}

@inproceedings{mairal2016end,
  title={End-to-end kernel learning with supervised convolutional kernel networks},
  author={Mairal, Julien},
  booktitle={Advances in neural information processing systems},
  pages={1399--1407},
  year={2016}
}

@inproceedings{batson2019noise2self,
  title={Noise2Self: Blind Denoising by Self-Supervision},
  author={Batson, Joshua and Royer, Loic},
  booktitle={International Conference on Machine Learning},
  pages={524--533},
  year={2019}
}

@article{d2020double,
  title={Double trouble in double descent: Bias and variance (s) in the lazy regime},
  author={d'Ascoli, St{\'e}phane and Refinetti, Maria and Biroli, Giulio and Krzakala, Florent},
  journal={arXiv preprint arXiv:2003.01054},
  year={2020}
}

@inproceedings{shaham2019singan,
  title={Singan: Learning a generative model from a single natural image},
  author={Shaham, Tamar Rott and Dekel, Tali and Michaeli, Tomer},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={4570--4580},
  year={2019}
}

@inproceedings{borle2019analyzing,
  title={Analyzing the quantum annealing approach for solving linear least squares problems},
  author={Borle, Ajinkya and Lomonaco, Samuel J},
  booktitle={International Workshop on Algorithms and Computation},
  pages={289--301},
  year={2019},
  organization={Springer}
}

@article{lacotte2019high,
  title={High-Dimensional Optimization in Adaptive Random Subspaces},
  author={Lacotte, Jonathan and Pilanci, Mert and Pavone, Marco},
  journal={arXiv preprint arXiv:1906.11809},
  year={2019}
}

@inproceedings{chowdhury2018iterative,
  title={An iterative, sketching-based framework for ridge regression},
  author={Chowdhury, Agniva and Yang, Jiasen and Drineas, Petros},
  booktitle={International Conference on Machine Learning},
  pages={988--997},
  year={2018}
}

@article{wang2017sketching,
  title={Sketching meets random projection in the dual: A provable recovery algorithm for big and high-dimensional data},
  author={Wang, Jialei and Lee, Jason D and Mahdavi, Mehrdad and Kolar, Mladen and Srebro, Nathan and others},
  journal={Electronic Journal of Statistics},
  volume={11},
  number={2},
  pages={4896--4944},
  year={2017},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}

@inproceedings{ozaslan2019iterative,
  title={Iterative Hessian Sketch with Momentum},
  author={Ozaslan, Ibrahim Kurban and Pilanci, Mert and Arikan, Orhan},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7470--7474},
  year={2019},
  organization={IEEE}
}

@Article{Ne03,
  title =	 {Properties of Highly Clustered Networks},
  author =	 {Newman, M. E. J.},
  doi =		 {10.1103/PhysRevE.68.026121},
  journal =	 {Phys. Rev. E},
  volume =	 {68},
  year =	 {2003},
  eid =		 {026121},
  pagetotal =	 6,
  month =	 aug,
}

@misc{clawpack,
  title =	 {Clawpack Software},
  author =	 {{Clawpack Development Team}},
  url =		 {http://www.clawpack.org},
  urldate =	 {2015/05/14},
  note =	 {Version 5.2.2},
  year =	 2015
}

@Misc{AMSMSC2010,
  title =	 {{Mathematics Subject Classification}},
  author =	 {{American Mathematical Society}},
  year =	 {2010},
  url =		 {http://www.ams.org/mathscinet/msc/msc2010.html},
  urldate =	 {2015/03/29},
}


@book{La86,
  author =	 "Leslie Lamport",
  title =	 "\LaTeX: A Document Preparation System",
  publisher =	 "Addison--Wesley",
  year =	 "1986",
  address =	 "Reading, MA"
}

@Book{MiGo04,
  author =	 {Frank Mittlebach and Michel Goossens},
  title =	 {The \LaTeX\ Companion},
  publisher =	 {Addison--Wesley},
  year =	 2004,
  edition =	 {2nd}}

@Book{GoVa13,
  author =	 {Golub, Gene H. and Van Loan, Charles F.},
  title =	 {Matrix Computations},
  publisher =	 {The Johns Hopkins University Press},
  address =	 {Baltimore},
  year =	 2013,
  edition =	 {4th}
}


@Misc{CalcI,
  author =	 {Paul Dawkins},
  title =	 {Paul's Online Math Notes: Calculus {I} --- Notes},
  url =               {http://tutorial.math.lamar.edu/Classes/CalcI/MeanValueTheorem.aspx},
  urldate =	 {2015-07-08}}

@Misc{amsmath,
  author =	 {{American Mathematical Society}},
  title =	 {User's Guide for the \texttt{amsmath} Package
                  (Version 2.0)},
  url =		 {ftp://ftp.ams.org/pub/tex/doc/amsmath/amsldoc.pdf},
  urldate =	 {2015-07-30},
  year =	 2002}

@Misc{shortmath,
  author =	 {Michael Downes},
  title =	 {Short Math Guide for {\LaTeX}},
  url =		 {ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf},
  urldate =	 {2015-07-30},
  year =	 2002}

@Misc{pgfplots,
  author =	 {Christian Feuers\"anger},
  title =	 {Manual for Package \texttt{PGFPLOTS}},
  month =	 may,
  year =	 2015,
  url =		 {http://sourceforge.net/projects/pgfplots}
}



==> defs.tex <==
% Colors
\definecolor{ddarkbrown}{rgb}{0.5,0.2,0.05} \definecolor{bbluegray}{rgb}{0.05,0,0.5}


% some traditional defintions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}

\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% Refs, etc
\newcommand{\refp}[1]{(\ref{#1})}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{{\mathbb R}}
\newcommand{\sreals}{\scriptsize{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\diam}{\mathop{\bf diam}}
\newcommand{\sphere}{{\mathbb S}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\NumRank}{\mathop{\bf NumRank}}
\newcommand{\NumCard}{\mathop{\bf NumCard}}
\newcommand{\Card}{\mathop{\bf Card}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
%XXX dumb question: do we not use \diag(...) to form diagonal or 
%block diagonal matrices?
\newcommand{\idm}{\mathbf{I}}

% probability stuff
\newcommand{\Expect}{\textstyle\mathop{\bf E}}
\newcommand{\Median}{\textstyle\mathop{\bf M}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
\newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
\newcommand{\QED}{~~\rule[-1pt]{6pt}{6pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\var}{\mathop{\bf var}}

\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\xopt}{x^{\rm opt}}

%the following ones seem way too specialized to be here...
%let's omve them to a new file called defs2.tex or something like that
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

% defs for cones & generalized inequalities
\newcommand{\geqK}{\mathrel{\succeq_K}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}

% From Alex
\newcommand{\realsp}{\mathbf{R}_+^n}
\newcommand{\intrealsp}{\int_{\mathbf{R}_+^n}}
\newcommand{\dirac}[1]{\mathbbm{1}_{\{#1\}}}



